Statistical Verification of Traffic Systems with Expected Differential Privacy

Traffic systems are multi-agent cyber-physical systems whose performance is closely related to human welfare. They work in open environments and are subject to uncertainties from various sources, making their performance hard to verify by traditional model-based approaches. Alternatively, statistical model checking (SMC) can verify their performance by sequentially drawing sample data until the correctness of a performance specification can be inferred with desired statistical accuracy. This work aims to verify traffic systems with privacy, motivated by the fact that the data used may include personal information (e.g., daily itinerary) and get leaked unintendedly by observing the execution of the SMC algorithm. To formally capture data privacy in SMC, we introduce the concept of expected differential privacy (EDP), which constrains how much the algorithm execution can change in the expectation sense when data change. Accordingly, we introduce an exponential randomization mechanism for the SMC algorithm to achieve the EDP. Our case study on traffic intersections by Vissim simulation shows the high accuracy of SMC in traffic model verification without significantly sacrificing computing efficiency. The case study also shows EDP successfully bounding the algorithm outputs to guarantee privacy.

==> Journal Sections/SDP_Challenges.tex <==
\section{\my{Standard differential privacy and challenges}} \label{sec:sdp}
% \my{Given algorithm $\mathscr{A}$ for~\eqref{eq:sprt_assertion}, it samples signals $\sigma_1, \sigma_2, \ldots$ from a probabilistic model $\mathcal{S}$ until its termination condition is satisfied; this sequence of samples is denoted as $\sigma_{1:\infty} = (\sigma_1, \sigma_2, \ldots)$. Meaning, $\mathscr{A}$ stops after a sample termination time $\tau_\mathscr{A} \in \nat$ before producing an output $o_\mathscr{A}$. Thus, the termination time and output can be treated as functions of $\sigma_{1:\infty}$ with $\tau_\mathscr{A}  (\sigma_{1:\infty})$ and $o_\mathscr{A}  (\sigma_{1:\infty})$, respectively.}

% Differential privacy aims to prevent malicious inference on $\sigma_{1:\infty}$. Roughly, Algorithm $\mathscr{A}$ is differentially private if an attacker cannot infer the value of $\sigma_i$ even if they can observe $(\tau_\mathscr{A} (\sigma_{1:\infty}), o_\mathscr{A}  (\sigma_{1:\infty}))$ and the values of the rest of the entries $\sigma_{-i}$ of $\sigma_{1:\infty}$, for any sequence $\sigma_{1:\infty}$ and entry $\sigma_i$ in $\sigma_{1:\infty}$.~\cite{dwork2008differential}. Clearly, for a deterministic Algorithm $\mathscr{A}$, the value of $\sigma_i$ can be inferred when the inverse of $\tau_\mathscr{A} (\cdot)$ and $o_\mathscr{A} (\cdot)$ is unique after knowing the value of $\sigma_{-i}$.

\my{Since $\mathscr{A}$ is deterministic, an intruder can infer the value of a single sample $\sigma_i \subseteq \sigma_{1:\infty}$ by obtaining the values of the remaining samples $\sigma_{-i} \subseteq \sigma_{1:\infty}$ and taking the inverse of $\tau_\mathscr{A}  (\sigma_{1:\infty})$ and $o_\mathscr{A}  (\sigma_{1:\infty})$. To achieve standard differential privacy, one common approach is to randomly execute $\mathscr{A}$ in slightly different ways for the same $\sigma_{1:\infty}$ to yield different observations. For a randomized algorithm $\mathscr{B}$ of $\mathscr{A}$, this prevents the intruder from taking the inverse of $\tau_{\mathscr{B}} (\cdot)$ and $o_{\mathscr{B}} (\cdot)$. However, the intruder can still infer the value of $\sigma_i$ by observing differences in $\tau_{\mathscr{B}}  (\sigma_{1:\infty})$ and $o_{\mathscr{B}}  (\sigma_{1:\infty})$ when $\sigma_{-i}$ is held constant and only $\sigma_i$ changes. This altered sequence of samples is denoted as $\sigma_{1:\infty}'$ and the Hamming distance $D_H$ between $\sigma_{1:\infty}$ and $\sigma_{1:\infty}'$ is 1 (i.e., $D_H (\sigma_{1:\infty}, \sigma_{1:\infty}') = 1$).}

\todo{Resume from here.}
\my{Differential privacy requires a bound on the worst case change in the probabilities of the random observations for two adjacent input sequences. If the change in distribution is smaller, then it is harder for the intruder to infer the change in the input. We apply the standard notion of differential privacy in \cite{dwork2008differential} to Algorithm~\ref{alg:1} of Section~\ref{sec:prelim} in the following definition.}


\my{\begin{definition} \label{def:differential privacy}
A randomized sequential algorithm $\mathscr{B}$ is $\varepsilon$-differentially private, if it holds that
\begin{align} 
&\mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}), o_{\mathscr{B}} (\sigma_{1:\infty}) \big) \in \mathcal{O} \Big) \notag
\\ &\leq e^{\varepsilon} \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}'), o_\mathscr{A} (\sigma_{1:\infty}') \big) \in \mathcal{O} \Big) \label{eq:standard differential privacy}
\end{align}
for any two adjacent input sequences $\sigma_{1:\infty}$ and $\sigma_{1:\infty}'$ and any $\mathcal{O} \subseteq \mathbb{N} \times \{H_\textrm{null}, H_\textrm{alt}\}$. 
\end{definition}}

\my{The standard approach to make deterministic algorithms differentially private is to randomize their outputs by the exponential algorithm~\cite{mcsherry2007mechanism}. However, we show below that the exponential algorithm cannot achieve the differential privacy from Definition~\ref{def:differential privacy} for the statistical model checking method shown in Algorithm~\ref{alg:1}.}

\my{For simplicity, consider only the observation of the termination time $\tau_\mathscr{A} (\sigma_{1:\infty})$. We can define the sensitivity of termination time to changes in any single entry by 
\begin{equation}
\delta_{\tau_\mathscr{A}} := \max_{D_H (\sigma_{1:\infty}, \sigma_{1:\infty}') = 1} \big| \tau_\mathscr{A} (\sigma_{1:\infty}) - \tau_\mathscr{A} (\sigma_{1:\infty}') \big|,
\end{equation}
i.e., the maximal difference in termination time for any two adjacent input sequences of sample signals $\sigma_{1:\infty}$ and $\sigma_{1:\infty}'$.}

\my{If the sensitivity $\delta_{\tau_\mathscr{A}}$ is finite, then the following exponential algorithm achieves differential privacy. The exponential mechanism states that  randomizing algorithm $\mathscr{A}$ to $\mathscr{B}$ such that the probability of terminating at step $k$ is 
\begin{equation} \label{eq:exponential mechanism}
\mathbb{P}_{\mathscr{B}} (\tau_{\mathscr{B}} = k) = \frac{e^{- \varepsilon |\tau_\mathscr{A} - k| / \delta_{\tau_\mathscr{A}}}}{\sum_{h \in \mathcal{H}} e^{- \varepsilon |\tau_\mathscr{A} - h| / \delta_{\tau_\mathscr{A}}}},
\end{equation}
where $\mathcal{H} \subseteq \nat$ is the set of possible values of $\mathscr{A}$, and $\mathbb{P}_{\mathscr{B}}$ means that the randomness should come from the algorithm $\mathscr{B}$ itself. The exponential mechanism~\eqref{eq:exponential mechanism} is $2 \varepsilon$-differentially private~\cite{mcsherry2007mechanism}, since for any two adjacent $\sigma_{1:\infty}$ and $\sigma_{1:\infty}'$, it holds by the definition of sensitivity that for any $k \in \nat$,
\begin{equation} \label{eq:1}
\frac{e^{- \varepsilon  |\tau_\mathscr{A} (\sigma_{1:\infty}) - k| / \delta_{\tau_\mathscr{A}}}}{e^{- \varepsilon  |\tau_\mathscr{A} (\sigma_{1:\infty}') - k| / \delta_{\tau_\mathscr{A}}}} \leq e^{\varepsilon |\tau_\mathscr{A} (\sigma_{1:\infty}) - \tau_\mathscr{A} (\sigma_{1:\infty}')| / \delta_{\tau_\mathscr{A}}} \leq e^{\varepsilon},
\end{equation}
where the first inequality holds by applying the triangle inequality. Since~\eqref{eq:1} holds for any $k$, we have
\begin{equation} \label{eq:2}
\frac{\sum_{h \in \mathcal{H}} e^{- \varepsilon  |\tau_\mathscr{A} (\sigma_{1:\infty}) - h| / \delta_{\tau_\mathscr{A}}}}{\sum_{h \in \mathcal{H}} e^{- \varepsilon  |\tau_\mathscr{A} (\sigma_{1:\infty}') - h| / \delta_{\tau_\mathscr{A}}}} \leq e^\varepsilon.
\end{equation}
Thus, the probability ratio satisfies
\begin{equation} \label{eq:3}
\frac{\mathbb{P}_{\mathscr{B}} \big( \tau_{\mathscr{B}}(\sigma_{1:\infty}) = k \big)}{\mathbb{P}_{\mathscr{B}} \big( \tau_{\mathscr{B}}(\sigma_{1:\infty}') = k \big)} \leq e^{2 \varepsilon}.
\end{equation}}


\my{The above technique depends critically on the boundedness of the sensitivity $\delta_{\tau_\mathscr{A}}$, which is generally true for non-sequential algorithms~\cite{mcsherry2007mechanism}. However, this condition is violated for Algorithm~\ref{alg:1}, as shown in Example~\ref{ex:counter}.}

% To achieve EDP, the termination time and output of \eqref{eq:sprt_test} should be randomized. This will be done by carefully adding a randomization algorithm to the termination conditions.

==> Journal Sections/smc.tex <==
\section{Statistical Model Checking for STL Specifications with Undetermined Test Function}
\label{sec:parametrized smc}

In practice, many specifications are given with undetermined test functions. For example, suppose the $\mathcal{S}$ is an autonomous electric car and the signal $\sigma = (\sigma_1, \sigma_2)$ is the velocity and battery level. The performance specification in signal temporal logic  
\begin{equation} \label{eq:ex2}
	(f_2 (\sigma_2) > 0) \ \mathcal{U}_{[0, 10]} \ (f_1 (\sigma_1) > 0)
\end{equation}
means within a time horizon of $10$, the car velocity should maintain $f_2 (\sigma_2) > 0$ before the battery level becomes $f_1 (\sigma_1) > 0$. This specification generalizes the specification in Example~\ref{ex:1} with the undetermined test functions $f = (f_1, f_2) \in \mathcal{F}$. They are customizable and may be different from car to car. For the manufacturer, a key problem is whether the satisfaction probability of the STL specification is greater than some given probability threshold $p \in [0,1]$ for any possible choice of $f \in \mathcal{F}$. 


\subsection{STL with Undetermined Test Functions} \label{sub:stl}

Formally, let $\varphi_f$ be an STL formula with undetermined test functions $f \in \mathcal{F}$ (like in~\eqref{eq:ex2}). We typically want to reason about the minimal/maximal satisfaction probability. To simplify the discussion, we focus on checking the minimal probability of $\sigma$ satisfying $\varphi_f$ is greater than some given probability threshold $p \in [0,1]$, i.e.,
\begin{equation} \label{eq:problem 2}
	\min_{f \in \mathcal{F}} \mathbb{P}_{\sigma \sim \mathcal{S}} ( \sigma \models \varphi_f ) = \min_{f \in \mathcal{F}} p_{\varphi_f} = \underline{p} > p
\end{equation}
where $\sigma$ is a random signal drawn from the probabilistic model $\mathcal{S}$. Maximal probabilities can be handled similarly via
$$\min_{f \in \mathcal{F}} \mathbb{P}_{\sigma \sim \mathcal{S}} ( \sigma \models \varphi_f ) > p \Longleftrightarrow \min_{f \in \mathcal{F}} \mathbb{P}_{\sigma \sim \mathcal{S}} ( \sigma \models \varphi_f ) \leq 1 - p.$$

To infer the correctness of the statement~\eqref{eq:problem 1} by statistical inference, we formulate it as a hypothesis testing problem
\begin{align} \label{eq:problem 2 ht}
& H_\textrm{null}: \underline{p} > p, \notag
\\ & H_\textrm{alt}: \underline{p} \leq p, 
\end{align}
where $H_\textrm{null}$ and $H_\textrm{alt}$ are the null and alternative hypotheses. Let 
$$\sigma_{1:N} = (\sigma_1, \ldots, \sigma_N)$$ 
be independent sample signals from the probabilistic model $\mathcal{S}$ (see Remark~\ref{rem:independent}). Now to check~\eqref{eq:problem 2 ht}, we evaluate the truth value of $\varphi$ on each sample signals $\sigma_i$ by $\varphi_f(\sigma_i)$, as defined in~\eqref{eq:varphi}. Each $\varphi(\sigma_i)$ is a binary random variable with parameter $p_{\varphi_f}$. 

Since the sample signals $\sigma_{1:N}$ are independent, the sum $\sum_{i \in [N]} \varphi_f (\sigma_{i}) \sim \mathrm{Binom} (N, p_{\varphi_f})$ obeys the binomial distribution. Thus, the satisfaction probability $p_{\varphi_f}$ can be approximated by the sample average $\sum_{i \in [N]} \varphi_f ( \sigma_{i})/N$ for each $f \in \mathcal{F}$. Accordingly, the minimal satisfactions probability $\min_{f \in \mathcal{F}} p_{\varphi_f}$ can be approximated by the minimal empirical satisfactions probability
\begin{equation} \label{eq:underline p}
\underline{p}_N = \frac{\min_{f \in \mathcal{F}} \sum_{i \in [N]} \varphi_f ( \sigma_{i})}{N}.
\end{equation}
Therefore, we define the statistical assertion for the statement~\eqref{eq:problem 2 ht} as
\begin{align} \label{eq:assert_2}
& \mathscr{A} \big( \sigma_{1:N} \big) = \begin{cases}
	H_\textrm{null}, &\text{ if } \underline{p}_N > p \\
	H_\textrm{alt}, &\text{ otherwise.}
\end{cases}
\end{align}
where $\underline{p}_N$ is defined in~\eqref{eq:underline p}. 


\subsection{Empirical Risk Minimization} 
\label{sub:erm}

To facilitate further discussion, let $\Omega$ be the set of all signals, $P$ be the unknown probability distribution of the sample signals $\sigma_1, \ldots, \sigma_N$, and 
\begin{equation} \label{eq:P_N}
P_N = \frac{1}{N} \sum_{i \in [N]} \delta_{\sigma_i} 
\end{equation}
be the empirical sample distribution, where $\delta$ is the Dirac delta function. Then, with a slight abuse of notations, we can write
\begin{align}
& \underline{p} = \min_{f \in \mathcal{F}} P(f) = \min_{f \in \mathcal{F}} \int_{\Omega} \varphi_f (\sigma) \d P,	
\\ & \underline{p}_N = \min_{f \in \mathcal{F}} P_N(f) = \min_{f \in \mathcal{F}} \int_{\Omega} \varphi_f (\sigma) \d P_N.
\end{align}

To ensure the assertion $\mathscr{A}$ is asymptotically accurate, i.e., $\mathscr{A}$ agrees with the ground truth of the problem~\eqref{eq:problem 2 ht} for $N \to \infty$, we make Assumption~\ref{ass:vc} that captures the complexity of the possibly-infinite function set $\mathcal{F}$. It generally holds on function sets with a finite number of parameters. By the Glivenko-Cantelli theorem, we have $P_N \to P$ in distribution for $N \to \infty$. With Assumption~\ref{ass:vc}, it holds that that $\underline{p}_N \to \underline{p}$ (see Remark~\ref{rem:Rademacher}).
\begin{assumption} \label{ass:vc}
The set of functions $\mathcal{F}$ has finite VC dimension~\cite{vapnik2000nature}.
\end{assumption}  


For statistical model checking, we need to derive quantitative bounds of the significance level of $\mathscr{A}$, i.e., the FP and FN ratios $\alpha_\textrm{FP}$ and $\alpha_\textrm{FN}$ for a finite $N$. For this goal, we use results from empirical risk minimization to capture the error of using the empirical statistic $\underline{p}_N$ in~\eqref{eq:assert_2} to approximate $\underline{p}$ in~\eqref{eq:problem 2}. To start with, the difference $|\underline{p}_N - \underline{p}|$ is bounded by the difference between $P$ and $P_n$.

\begin{lemma} \label{lem:1}
It holds that 
$$|\underline{p}_N - \underline{p}| \leq \Vert P_N - P \Vert_\mathcal{F}$$ 
where 
$$\Vert P_N - P \Vert_\mathcal{F} = \max_{f \in \mathcal{F}} \big| \int_{\Omega} \varphi_f (\sigma) \d (P-P_N) \big|$$
\end{lemma}

\begin{proof}
Let 
\begin{align*}
& f^* = \textrm{argmin}_{f \in \mathcal{F}} P(f),
\\ & f_N^* = \textrm{argmin}_{f \in \mathcal{F}} P_N(f).
\end{align*}
Then
\begin{align*}
\underline{p}_N - \underline{p} & = P_N (f_N^*) - P (f^*) 
\\ & = (P_N (f_N^*) - P_N (f^*)) + (P_N (f^*) - P (f^*)) 
\\ & \leq P (f^*) - P (f^*) \leq \Vert P_N - P \Vert_\mathcal{F}. 
\end{align*}
noting that $P_N (f_N^*) - P_N (f^*) \leq 0$. Similarly, 
\begin{align*}
\underline{p}_N - \underline{p} & = P_N (f_N^*) - P (f^*) 
\\ & = (P_N (f_N^*) - P (f_N^*)) + (P (f_N^*) - P (f^*)) 
\\ & \geq P (f^*) - P (f^*) \geq - \Vert P_N - P \Vert_\mathcal{F}. 
\end{align*}
Thus, the lemma holds.
\end{proof}

Due to the randomness in the sample signals $\sigma_{1:N}$, the difference between $\Vert P_N - P \Vert_\mathcal{F}$ is a random variable. Its expected value can be estimated by the Rademacher average, as proved in~\cite{gine1984limit}.

\begin{lemma} \label{lem:2}
It holds that 
$$\mathbb{E}_{\sigma_{1:N}} \Vert P_N - P \Vert_\mathcal{F} \leq 2 \mathbb{E}_{\sigma_{1:N}} \mathcal{R}_N (\mathcal{F})$$ 
\begin{equation*} \label{eq:Rad}
\mathcal{R}_N (\mathcal{F}) = \mathbb{E}_{\eta_{1:N}} \max_{f \in \mathcal{F}} \Big| \frac{1}{N}\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i) \Big|
\end{equation*}
where $\eta_{1}, \ldots, \eta_n$ are i.i.d. Rademacher random variables with probability distribution 
$$
\eta_i = \begin{cases}
1, & \text{with probability } 0.5, \\
-1, & \text{with probability } 0.5,
\end{cases}
$$
and $\mathcal{R}_N (\cdot)$ is the Rademacher average.
\end{lemma}


By concentration inequalities, the bound of  the difference between $\Vert P_N - P \Vert_\mathcal{F}$ is a random variable. Its expected value can be estimated by the Rademacher average.


\begin{lemma} \label{lem:3}
It holds with probability at most $e^{- \frac{2 \delta^2 N}{9}}$ that 
$$|\underline{p}_N - \underline{p}| \geq 2 \mathcal{R}_N (\mathcal{F}) + \delta.$$
\end{lemma}

\begin{proof} 
By Lemma~\ref{lem:1} and~\ref{lem:2}, we have
\begin{align*}
& \mathbb{E}_{\sigma_{1:N}} \Big( |\underline{p}_N - \underline{p}| - 2 \mathcal{R}_N (\mathcal{F}) \Big)
\\ & \qquad \leq \mathbb{E}_{\sigma_{1:N}} \Big(\Vert P_N - P \Vert_\mathcal{F} - 2 \mathcal{R}_N (\mathcal{F}) \Big)  \leq 0
\end{align*}
Now we apply McDiarmid's inequality. Consider the mapping from the sample signals $\sigma_{1:N}$ to the approximation error $|\underline{p}_N - \underline{p}| - 2 \mathcal{R}_N (\mathcal{F})$. For any two values of sample signals $\sigma_{1:N}$ and $\sigma_{1:N}'$ that differ in only one entry, it is bounded by 
\begin{align*}
& \Big| \Big(|\underline{p}_N - \underline{p}| - 2 \mathcal{R}_N (\mathcal{F}) \Big) - \Big(|\underline{p}_N' - \underline{p}| - 2 \mathcal{R}_N' (\mathcal{F}) \Big) \Big| 
\\ &  \leq \Big| |\underline{p}_N - \underline{p}| - |\underline{p}_N' - \underline{p}| \Big| + 2 \Big| \mathcal{R}_N (\mathcal{F}) - \mathcal{R}_N' (\mathcal{F}) \Big| 
\\ &  \leq \Big| \underline{p}_N - \underline{p}_N'  \Big| + 2 \Big| \mathcal{R}_N (\mathcal{F}) - \mathcal{R}_N' (\mathcal{F}) \Big| \leq \frac{3}{N}, 
\end{align*}
because
\begin{align*}
&  \Big| \underline{p}_N - \underline{p}_N'  \Big| 
\\ &  = \Big| \frac{\min_{f \in \mathcal{F}} \sum_{i \in [N]} \varphi_f ( \sigma_{i} )}{N} - \frac{\min_{f \in \mathcal{F}} \sum_{i \in [N]} \varphi_f ( \sigma_{i}' )}{N} \Big|
\\ &  \leq \Big| \min_{f \in \mathcal{F}} \frac{\sum_{i \in [N]} \varphi_f ( \sigma_{i}' )}{N} - \frac{\sum_{i \in [N]} \varphi_f ( \sigma_{i})}{N} \Big| \leq  \frac{1}{N}
\end{align*}
and 
\begin{align*}
& \Big| \mathcal{R}_N (\mathcal{F}) - \mathcal{R}_N' (\mathcal{F}) \Big| =
\\ & \Big| \mathbb{E}_{\eta_{1:N}} \max_{f \in \mathcal{F}} \big| \frac{\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i)}{N}  \big| - \max_{f \in \mathcal{F}} \big| \frac{\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i')}{N}  \big| \Big|
\\ &  \leq \Big| \mathbb{E}_{\eta_{1:N}} \max_{f \in \mathcal{F}} \big| \frac{\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i)}{N}  \big| - \big| \frac{\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i')}{N}  \big| \Big|
\\ &  \leq \Big| \mathbb{E}_{\eta_{1:N}} \max_{f \in \mathcal{F}} \big| \frac{\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i)}{N}  - \frac{\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i')}{N}  \big| \Big| \leq  \frac{1}{N}
\end{align*}
Thus, by McDiarmid's inequality to $|\underline{p}_N - \underline{p}| - 2 \mathcal{R}_N (\mathcal{F})$, we have 
\begin{align*}
& \mathbb{P} \big( |\underline{p}_N - \underline{p}| - 2 \mathcal{R}_N (\mathcal{F}) \geq \delta \big) \leq 
\\ & \mathbb{P} \Big( |\underline{p}_N - \underline{p}| - 2 \mathcal{R}_N (\mathcal{F}) - \mathbb{E}_{\sigma_{1:N}} \big( |\underline{p}_N - \underline{p}| - 2 \mathcal{R}_N (\mathcal{F}) \big) \geq \delta \Big) 
\\ & \leq e^{- \frac{2 \delta^2 N}{9}}.
\end{align*}
Thus, the lemma holds.
\end{proof}

\begin{remark} \label{rem:Rademacher}
When Assumption~\ref{ass:vc} holds, the Rademacher average $\mathcal{R}_N (\mathcal{F}) \to 0$ as $N \to \infty$~\cite{vapnik2000nature}. So Lemma~\eqref{lem:3} implies that $\underline{p}_N \to \underline{p}$, i.e., the assertion $\mathscr{A}$ agrees with the ground truth of the problem~\eqref{eq:problem 2 ht} almost surely.
\end{remark}




\subsection{Statistical Model Checking} 
\label{sub:smc}

We now develop a sequential algorithms for the hypotheses testing problem~\eqref{eq:problem 2 ht}. By Lemma~\ref{lem:3}, for a desired significance level $\alpha > 0$, the minimal satisfaction probability $\underline{p}$ in~\eqref{eq:problem 2 ht} is contained by the confidence interval.
\begin{equation} \label{eq:confidence interval}
\underline{p} \in \big( \underline{p}_N - d_N, \ \underline{p}_N + d_N \big),
\end{equation}
\begin{equation} \label{eq:d}
d_N = 2 \mathcal{R}_N (\mathcal{F}) + \sqrt{- \frac{9 \ln \alpha}{2 N}}
\end{equation}
where $\mathcal{R}_N (\mathcal{F})$ is given by~\eqref{eq:Rad}. Thus, if $\underline{p}_N + d_N < p$, then we can assert that 
$\min_{f \in \mathcal{F}} p_{\varphi_f} < p$ with the significance level less than $\alpha$. Similarly, if $\underline{p}_N - d_N > p$, then we can assert that $\min_{f \in \mathcal{F}} p_{\varphi_f} > p$ with the significance level less than $\alpha$. Otherwise, we keep on drawing new samples. Namely, the assertion is
\begin{equation} \label{eq:assert_2}
\mathscr{A} \big( \sigma_1, \ldots, \sigma_N \big) = \begin{cases}
H_\textrm{null}, & \text{ if } \underline{p}_N - d_N > p \\
H_\textrm{alt}, & \text{ if } \underline{p}_N + d_N < p \\
\text{continue}, & \text{ otherwise.}
\end{cases}
\end{equation}
This procedure is summarized by Algorithm~\ref{alg:2}. 

To ensure the termination and accurate of Algorithm~\ref{alg:2}, we introduce Assumption~\ref{as:indifference 2}.

\begin{assumption} \label{as:indifference 2}
It holds that $\underline{p} \neq p$ in~\eqref{eq:problem 2}.
\end{assumption}

\begin{remark} \label{lem:5}
Similar in spirit with Remark~\ref{rem:2}, by Assumption~\ref{as:indifference 2}, we do not distinguish between checking $\underline{p} > p$ or checking $\underline{p} \geq p$ in~\eqref{eq:problem 2}. In addition, the maximal satisfaction probabilities can be checked via the negation of minimal satisfaction probabilities in~\eqref{eq:problem 2}. For example, 
\begin{align*}
\max_{f \in \mathcal{F}} p_{\varphi_f} < p \ & \Longleftrightarrow \ \min_{f \in \mathcal{F}} p_{\neg \varphi_f} \geq 1 - p 
\\ & \Longleftrightarrow \ \min_{f \in \mathcal{F}} p_{\neg \varphi_f} > 1 - p.
\end{align*} 
\end{remark}

With Assumption~\ref{as:indifference 2}, the termination and accurate of Algorithm~\ref{alg:2} is ensured by Theorem~\ref{thm:1}.

\begin{algorithm}[!t]
\caption{SMC of $\min_{f \in \mathcal{F}} \mathbb{P}_{\sigma \sim \mathcal{S}} ( \sigma \models \varphi_f ) > p$.\label{alg:2}}

\begin{algorithmic}[1]
\Require System $\mathcal{S}$ and desired significance level $\alpha$.

\State $N \gets 0$.

\While{True}

\State $N \gets N + 1$

\State Draw sample signal $\sigma_N$ from $\mathcal{S}$

\State $\underline{p}_N = \frac{1}{N} \min_{f \in \mathcal{F}} \sum_{i \in [N]} \varphi_f ( \sigma_{i})$

\State $\mathcal{R}_N \gets \mathbb{E}_{\eta_{1:N}} \max_{f \in \mathcal{F}} \Big| \frac{1}{N}\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i) \Big|$

\State $d_N \gets 2 \mathcal{R}_N + \sqrt{- \frac{9 \ln \alpha}{2 N}}$

\If {$\underline{p}_N - d_N > p$} Return $H_\textrm{null}$

\ElsIf {$\underline{p}_N + d_N < p$} Return $H_\textrm{alt}$

\Else \ Continue

\EndIf 

\EndWhile
\end{algorithmic}
\end{algorithm}


\begin{theorem} \label{thm:1}
When $\underline{p} \neq p$ in~\eqref{eq:problem 2}, Algorithm~\ref{alg:2} terminates with probability $1$ and its return agrees with the ground truth of~\eqref{eq:problem 2} with probability at least $1-\alpha$.
\end{theorem}

\begin{proof}
{\bf Termination.} By Remark~\ref{rem:Rademacher}, we have $\mathcal{R}_N \to 0$ and $\underline{p}_N \to \underline{p}$ as $N \to \infty$. The former implies 
$$d_N = 2 \mathcal{R}_N + \sqrt{- \frac{9 \ln \alpha}{2 N}} \to 0.$$ 
The latter implies 
$$\underline{p}_N - p \to \underline{p} - p \neq 0.$$
Thus, $d_N < |p - p_N|$, i.e., the algorithm terminates for sufficiently large $N$.   

\noindent {\bf Probabilistic Correctness.} Consider the probabilistic events 
\begin{itemize}
	\item $\mathcal{T}$: The return of Algorithm~\ref{alg:2} agrees with the ground truth. 
	\item $\mathcal{T}_N$: The assertion~\eqref{eq:assert_2} agrees with the ground truth for the $N$ iteration.
\end{itemize}
Then
$\mathbb{P} (\mathcal{T}) = \sum_{i \in \nat} \mathbb{P} (\mathcal{T}_i) \mathbb{P} (N = i)$. By construction of the significance intervals, we have $\mathbb{P} (\mathcal{T}_i) > 1 - \alpha$ for any $i \in \nat$. In addition, by {\bf Termination}, we have $\sum_{i \in \nat} \mathbb{P}(\tau = i) = 1$. Thus, $\mathbb{P}(A) \geq 1 - \alpha_d$.
\end{proof}


\begin{remark} \label{lem:related}
By allowing the undetermined test function from a possibly infinite set $\mathcal{F}$, Algorithm~\ref{alg:2} simultaneously checks a possibly infinite set of STL formulas. It generalizes most previous works that focus on single STL formulas~\cite{legay2010statistical,agha2018survey}. Comparing previous work on statistical model checking for STL formula sets~\cite{wang2020probabilistic}, this method does not require the monotonicity condition on the STL formula sets. Finally, the condition $\underline{p} \neq p$ in Theorem~\ref{thm:1} is similar in spirit with~\cite{zarei2020statistical} to ensure the termination and probabilistic correctness of the statistical model checking algorithm.
\end{remark}


% \begin{remark} \label{lem:5}
% Similar in spirit with Remark~\ref{rem:2}, by the condition $\underline{p} \neq p$ in Theorem~\ref{thm:1}, we do not distinguish between checking $\underline{p} > p$ or checking $\underline{p} \geq p$ in~\eqref{eq:problem 2}. In addition, checking maximal satisfaction probabilities

% $\underline{p} < p$ or $\underline{p} \leq p$ is equivalent to checking $p_{\neg \varphi} \geq 1 - p$ or $p_{\neg \varphi} > 1 - p$. Thus, the method for checking $p_\varphi > p$ applies to the other three cases.
% \end{remark}






==> adp.tex <==
\section{Expected differential privacy} \label{sec:expected differential privacy}

Section III-\ref{sub:Laplace} has shown that the exponential mechanism cannot achieve the standard differential privacy (Definition~\ref{def:differential privacy}) for the statistical model checking Algorithm~\ref{alg:1}. In this section, we proposed a new notion called expected differential privacy, which is weaker than the standard one. We will show that expected differential privacy is achievable by a new type of exponential mechanism in Section \ref{sec:algorithm}.

One assumption that we make in this paper that has not been considered in standard differential privacy (Definition~\ref{def:differential privacy}) is that the sequences of signals that the algorithm processes
% $\sigma_{1:\infty}$ and $\sigma_{1:\infty}'$ 
are independently drawn from an underlying probability distribution. This is the probability model $\mathcal{S}$. This is a stronger assumption than the arbitrarily-valued static databases assumed in the literature of differential privacy~\cite{dwork2008differential}.
Such a stronger assumption helps in defining a relaxed notion of privacy that is based on limiting the change of the {\em average} of the algorithm's output over the {\em distribution} of input sequences with respect to arbitrary changes of an arbitrary entry. In contrast, standard differential privacy is based on limiting the change of the algorithm's output for {\em any} input with respect to arbitrary changes of any of the input's entries. 
%most probable input sequences to an algorithm, instead of all possible inputs.
In the case of Example~\ref{ex:counter}, 
% while achieving differential privacy is challenging, 
as we will show in this section, the average termination time of Algorithm~\ref{alg:1} over the distribution of input sequences is bounded. Thus, the probability that an input leads to an infinite termination time as the one shown in Example~\ref{ex:counter} is negligible.



% Particularly for Algorithm~\ref{alg:1}, the significance level $\alpha$ of statistical model checking is usually taken to be $\ll 1$. Thus, the termination time $K_1$ of Algorithm~\ref{alg:1} in Example~\ref{eq:ex2} is $\gg 1$, so the probability of sampling the sequences in Example~\ref{ex:counter} is almost $0$. 
% by inequalities~\eqref{eq:K_1} the probability of sampling the sequences in Example~\ref{ex:counter} is almost $0$. 
% Hence, even though Example~\ref{ex:counter} could occur theoretically, it is very unlikely to happen in practice that the two sequences happen to be sampled by Algorithm~$\mathscr{A}$ and the intruder observing its outputs. This motivates us to take the probability distribution generating the sequences into account for differential privacy.  


By Definition~\ref{def:differential privacy}, if a randomized sequential algorithm $\mathscr{B}$ is differentially private, the difference in the probability of the observations $(\tau_{\mathscr{B}} (\sigma_{1:\infty}), o_{\mathscr{B}} (\sigma_{1:\infty}))$ should be bounded under the change of a single entry $\sigma_n$ for any input sequence $\sigma_{1:\infty}$. 
However, under the assumption in this paper, all the sample signals in $\sigma_{-n}$ are drawn independently from the probabilistic model $\mathcal{S}$. We build on this assumption and propose an expected version of the standard differential privacy (Definition~\ref{def:differential privacy}) that requires the boundedness of the sensitivity of the average output and termination time.

% to hold in  values for $\sigma_{-i}$. 
%instead of requiring Definition~\ref{def:differential privacy} hold for any values of $\sigma_{-i}$, 
% when the significance level $\alpha$ is small enough. This implies 
% that the number of samples used by $\mathscr{B}$ (i.e., $\tau_{\mathscr{B}}$) is sufficiently large.


% \todo{I think I now understand more what you mean. I think it still needs a bit of clarification though for the general audience. It is not clear when you say "hardly noticeable".}

% \hussein{Are the values of $\sigma_n$ and $\sigma_n'$ fixed in the following definition? Or they follow the model/system probability distribution? The following definition is missing this detail/quantifier}
% A randomized sequential algorithm $\mathscr{B}$ is $\varepsilon$-expectedly differentially private if it achieves $\varepsilon$-differential privacy with high probability when $\alpha$ is small enough, as formally defined below.


% \begin{definition} \label{def:expected differential privacy}
% A randomized sequential algorithm $\mathscr{B}$ is $\varepsilon$-expectedly differentially private if
% \begin{align} 
% & \mathbb{P}_{\sigma_{-n}} \bigg( 
% \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}), o_{\mathscr{B}} (\sigma_{1:\infty}) \big) \in \mathcal{O} \Big) \notag
% \\ & \qquad \leq e^{\varepsilon} \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}'), o_{\mathscr{B}} (\sigma_{1:\infty}') \big) \in \mathcal{O} \Big)
% \bigg) \to 1, \label{eq:def 3}
% \end{align}
% as the significance level $\alpha \to 0$, i.e., 
% for any $\beta \in (0,1]$, there exists an $\alpha_0 > 0$ such that for all $\alpha < \alpha_0$,  
% \begin{align*} 
% & \mathbb{P}_{\sigma_{-n}} \bigg( 
% \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}), o_{\mathscr{B}} (\sigma_{1:\infty}) \big) \in \mathcal{O} \Big) \notag
% \\ & \qquad \leq e^{\varepsilon} \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}'), o_{\mathscr{B}} (\sigma_{1:\infty}') \big) \in \mathcal{O} \Big)
% \bigg) > 1 - \beta, 
% \end{align*}
% for any $ n \in \nat$, any $\mathcal{O} \subseteq \mathbb{N} \times \{H_\textrm{null}, H_\textrm{alt}\}$, and any pair of signals $\sigma_n$ and $\sigma'_n$, where $\sigma_{-n}$ is a random sequence of signals obeying the distribution of the probabilistic model $\mathcal{S}$ and $\sigma'_{-n} := \sigma_{-n}$.
% \end{definition}


% Definition~\ref{def:expected differential privacy} shows that the standard differential privacy implies the expected differential privacy, as the condition of Definition~\ref{def:expected differential privacy} can be derived from the condition of Definition~\ref{def:differential privacy}.


% %Checking whether a randomized algorithm $\mathscr{B}$ satisfies Definition~\ref{def:expected differential privacy} requires taking the limit $\tau_{\mathscr{B}} (\sigma_{1:\infty}), \tau_{\mathscr{B}} (\sigma_{1:\infty}') \to \infty$. To avoid this, 
% We provide the following sufficient condition for expected differential privacy. 
% % This condition focuses on the expected values of the random observations with respect to the sample signals.
% It requires that changing the value of an arbitrary $n^\mathit{th}$ signal can only change the expected values of the random observations slightly.


\begin{definition} \label{def:expected differential privacy}
Denote $\{H_\textrm{null}, H_\textrm{alt}\}$ by $\{1, 0\}$. 
A randomized sequential algorithm $\mathscr{B}$ is $\varepsilon$-expectedly differentially private if
%for a random sequence of signals $\sigma_{1:\infty}$ from the probabilistic model $\mathcal{S}$, it holds that 
\begin{align} 
&\mathbb{P}_{\mathscr{B}} \Big( \mathbb{E}_{\sigma_{-n}} \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}), o_{\mathscr{B}} (\sigma_{1:\infty}) \big) \in \mathcal{O} \Big) \notag
\\ & \leq e^{\varepsilon} \mathbb{P}_{\mathscr{B}} \Big( \mathbb{E}_{\sigma'_{-n}} \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}'), o_{\mathscr{B}} (\sigma_{1:\infty}') \big) \in \mathcal{O} \Big),
\label{eq:lemma 1}
\end{align}
for any $n \in \nat$, any $\mathcal{O} \subseteq \mathbb{N} \times \{1, 0\}$, and any pair of signals $\sigma_n$ and $\sigma'_n$, where $\sigma_{-n}$ and $\sigma'_{-n}$ are random sequences with i.i.d. entries following the probabilistic model $\mathcal{S}$.
We say that $\mathscr{B}$ is $\varepsilon$-expectedly differentially private {\em in termination time} if 
\begin{align} 
\mathbb{P}_{\mathscr{B}} \Big( \mathbb{E}_{\sigma_{-n}} \tau_{\mathscr{B}} (\sigma_{1:\infty}) \in \mathcal{O} \Big) \leq e^{\varepsilon} \mathbb{P}_{\mathscr{B}} \Big( \mathbb{E}_{\sigma'_{-n}} \tau_{\mathscr{B}} (\sigma_{1:\infty}') \in \mathcal{O} \Big), \label{eq:edp termination time}
\end{align}
for any $\mathcal{O} \subseteq \mathbb{N}$, $\sigma_n$, and $\sigma_n'$. 
\end{definition}

The expected differential privacy (Definition \ref{def:expected differential privacy}) is weaker than the standard one (Definition \ref{def:differential privacy}) since the condition of the latter \eqref{eq:standard differential privacy} implies the former \eqref{eq:lemma 1} by taking the expected values $\mathbb{E}_{\sigma_{-n}} \mathbb{E}_{\sigma'_{-n}}$  on both sides of the equation, i.e., 
\begin{align*}
& \mathbb{E}_{\sigma_{-n}} \mathbb{E}_{\sigma'_{-n}} \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}), o_{\mathscr{B}} (\sigma_{1:\infty}) \big) \in \mathcal{O} \Big)
\\ & \leq e^{\varepsilon} \mathbb{E}_{\sigma_{-n}} \mathbb{E}_{\sigma'_{-n}} \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}'), o_{\mathscr{B}} (\sigma_{1:\infty}') \big) \in \mathcal{O} \Big),
\end{align*}
for any $\mathcal{O} \subseteq \mathbb{N}$, $\sigma_n$, and $\sigma_n'$. This implies that
\begin{align*}
& \mathbb{E}_{\sigma_{-n}} \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}), o_{\mathscr{B}} (\sigma_{1:\infty}) \big) \in \mathcal{O} \Big)
\\ & \leq e^{\varepsilon} \mathbb{E}_{\sigma'_{-n}} \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}'), o_{\mathscr{B}} (\sigma_{1:\infty}') \big) \in \mathcal{O} \Big).
\end{align*}
Note that 
\begin{align*}
& \mathbb{E}_{\sigma_{-n}} \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}), o_{\mathscr{B}} (\sigma_{1:\infty}) \big) \in \mathcal{O} \Big)
\\ & = \mathbb{E}_{\sigma_{-n}} \mathbb{E}_{\mathscr{B}} \ \textbf{I} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}), o_{\mathscr{B}} (\sigma_{1:\infty}) \big) \in \mathcal{O} \Big)
\\ & = \mathbb{E}_{\mathscr{B}} \mathbb{E}_{\sigma_{-n}}  \ \textbf{I} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}), o_{\mathscr{B}} (\sigma_{1:\infty}) \big) \in \mathcal{O} \Big)
\\ & \leq e^{\varepsilon} \mathbb{E}_{\sigma'_{-n}} \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}'), o_{\mathscr{B}} (\sigma_{1:\infty}') \big) \in \mathcal{O} \Big),
\end{align*}
where $\textbf{I}(\cdot)$ is the indicator function and $\mathbb{E}_{\sigma_{-n}}$ and $\mathbb{E}_{\mathscr{B}}$ commute by Fubini's Theorem. Thus, we can flip $\mathbb{E}_{\sigma_{-n}}$ and $\mathbb{P}_{\mathscr{B}}$ (or $\mathbb{E}_{\sigma'_{-n}}$ and $\mathbb{P}_{\mathscr{B}}$) to derive the following inequality:
\begin{align*}
&  \mathbb{P}_{\mathscr{B}} \Big( \mathbb{E}_{\sigma_{-n}} \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}), o_{\mathscr{B}} (\sigma_{1:\infty}) \big) \in \mathcal{O} \Big)
\\ & \leq e^{\varepsilon} \mathbb{P}_{\mathscr{B}} \Big( \mathbb{E}_{\sigma'_{-n}} \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}'), o_{\mathscr{B}} (\sigma_{1:\infty}') \big) \in \mathcal{O} \Big).
\end{align*}






==> algorithm.tex <==
% \section{Preliminaries on Statistical Model Checking} \label{sec:prelim}
\section{Expected Differential Privacy for Statistical Model Checking}
\label{sec:algorithm}

% Real-world cyber-physical systems are typically subject to uncertainty in their parameters from different sources, e.g., thermal fluctuations in sensors/actuators. The probabilistic uncertainty is expressible by random variables drawn from probabilistic distributions, which may be unknown. For example, the uncertainty in the sensor readings can be expressed by the addition of a random noise. Such uncertainties can be captured by a probabilistic model. A key problem for the probabilistic model is whether a specification holds on a random system path with probability above some given threshold. Such a problem can be solved with provable probabilistic guarantees by statistical model checking. Below, we summarize previous work on statistical model checking algorithms based on sequentially probability ratio tests~\cite{legay2010statistical,agha2018survey}.

\subsection{Statistical model checking \my{and sequential probability ratio test}} \label{sub:smc}

Consider a random signal $\sigma$ from an arbitrary model $\mathcal{S}$. The goal of SMC is to check the probability of $\sigma$ satisfying a specification $\varphi$ being greater than some given threshold $p \in [0,1]$,
\begin{equation} \label{eq: SMC}
	\mathbb{P}_{\sigma \sim \mathcal{S}} ( \sigma \models \varphi ) = p_\varphi > p,
\end{equation}
where $\models$ means ``to satisfy'' and $p_\varphi$ is the satisfaction probability of $\varphi$ on $\mathcal{S}$. 

Formally, $\varphi$ is expressed by signal temporal logic (STL)~\cite{maler2004monitoring}, which is an extension of linear temporal logic by analyzing real-time and real-value systems in addition to discrete-time and Boolean systems. This allows SMC to work with continuous or hybrid systems.
\todo{Include semantics and syntax of STL. Come back to rephrase these paragraphs.}
% , which contains a simple set of syntactic rules to describe the change of real-valued system variables in continuous time.

The syntax of STL specifications is defined recursively by:
\[
\varphi :=
f (\sigma) \geq 0
\mid \neg \varphi
\mid \varphi \land \varphi
\mid \varphi \ \mathcal{U}_{[t_1,t_2]} \ \varphi,
\]
where $\sigma: \nnreal \to \real^n$ is a real-valued signal
% (i.e., a vector of real-valued system variables that changes over time)
, $f: \real^n \to \real$ is a real-valued function of the signal, and $[t_1, t_2]$ is a time interval with $t_2 > t_1 \geq 0$. Strictly speaking, $t_1$ and $t_2$ should be rational-valued or infinity. By recursively applying these syntactic rules, we can write arbitrarily complex STL specifications to express general specifications of interest.


Given any STL specification $\varphi$, we can define whether a signal $\sigma$ satisfies it or not, written as $\sigma \models \varphi$ or $\sigma \not\models \varphi$, using the following semantic rules: 
\begin{align*}
& \sigma \models f (\sigma) \geq 0  & \ \Leftrightarrow \ &   f(\sigma(0)) \geq 0 \\
& \sigma \models \neg \varphi  & \ \Leftrightarrow \ &  \sigma \not\models \varphi \\
& \sigma \models \varphi \land \psi  & \ \Leftrightarrow \ &  \sigma \models \varphi \land \sigma \models \psi \\
& \sigma \models \varphi \ \mathcal{U}_{[t_1,t_2]} \ \psi & \ \Leftrightarrow \ &  \exists t \in [t_1, t_2] \text{ such that } \sigma^{(t)} \models \psi \\
& & & \land \forall t' < t, \sigma^{(t')} \models \varphi
\end{align*}
where $\sigma^{(t)}$ denotes the $t$-shift of $\sigma$, defined by $\sigma^{(t)}(t') = \sigma(t + t')$ for any $t' \in \nnreal$. 
The first rule means that $\sigma$ satisfies $f (\sigma) \geq 0$ if and only if the initial value of $\sigma$ at time $t=0$ satisfies $f (\sigma(0)) \geq 0$. The fourth rule defined the ``until'' temporal operator; it means that $\sigma$ satisfies $\varphi \ \mathcal{U}_{[t_1,t_2]} \ \psi$ if and only if $\sigma$ satisfies $\varphi$ at all time instants before $t$ until it satisfies $\psi$ exactly at time $t$ for some $t \in [t_1,t_2]$. 

Using the STL syntax and semantics, we can define other temporal operators such as ``finally'' (or ``eventually'') and ``always'', written as $\Diamond$ and $\square$. Specifically, 
$\Diamond_{[t_1,t_2]} \varphi = \mathtt{True} \ \mathcal{U}_{[t_1,t_2]} \ \varphi$ 
means the property $\varphi$ finally holds; and 
$\square_{[t_1,t_2]} \varphi = \neg (\Diamond_{[t_1,t_2]} \neg\varphi)$ 
means the property $\varphi$ always holds. In addition, although only the inequality symbol ``$>$'' is included in the STL syntax, we can express other inequalities symbols via the semantics. For example, $f (\sigma) > 0$ can be expressed by $ \neg \big( {-} f (\sigma) \geq 0 \big)$. Below, we will also use these operators or symbols in STL specifications.   

% \begin{example} \label{ex:1}
% Suppose $\sigma = (\sigma_1, \sigma_2)$ where $\sigma_1$ and $\sigma_2$ are the velocity and battery level of an electric vehicle. Then the specification
% $$(\sigma_1 > 5) \ \mathcal{U}_{[0, 10]} \ (\sigma_2 < 0.2)$$
% means the car velocity should be greater than $5$ before the battery level drops below $0.2$ within $10$ time units. 
% \end{example}




% \subsection{Sequential probability ratio test} \label{sub: sprt}

SMC handles \eqref{eq: SMC} as a hypothesis testing problem
\begin{align} \label{eq: hypothesis testing}
H_\textrm{null}: p_\varphi > p, \quad
H_\textrm{alt}: p_\varphi \leq p, 
\end{align}
where $H_\textrm{null}$ and $H_\textrm{alt}$ are the null and alternative hypotheses respectively. Then, it draws sample signals $\sigma_1, \sigma_2, \ldots$ from $\mathcal{S}$ to verify whether $H_\textrm{null}$ or $H_\textrm{alt}$ holds. Correlated sampling has been shown to improve SMC efficiency, but it requires some knowledge of the system dynamics~\cite{wang2018statisticala,wang2019statistical}. A traffic intersection is a highly-complex system that depends on many factors. Therefore, this work focuses on independent sampling, which can handle general black-box systems~\cite{agha2018survey, legay2010statistical}.
%As with previous work~\cite{legay2010statistical,agha2018survey}, we focus on samples that are drawn independently. 

% \begin{remark} \label{rem:independent}
% It has been shown that correlated samples can improve the efficiency of statistical model checking~\cite{wang2018statisticala,wang2019statistical}. However,  using correlated samples requires at least partial knowledge of the system dynamics to implement. On the other hand, independent sampling can apply to general black-box systems.
% \end{remark}

SMC examines the correctness of $\varphi$ on each sample signal $\sigma_i$ as the following Boolean
% This process can be performed automatically by existing model checking algorithms from~\cite{maler2004monitoring,roohi2018revisiting}. With a slight abuse of notation, we represent ``True'' and ``False'' by $1$ and $0$ and define the truth values by
\begin{equation} \label{eq:varphi}
\varphi(\sigma_i) = \begin{cases}
1, & \sigma_i \models \phi, \\
0, &\text{ otherwise.}
\end{cases}
\end{equation}
% Each $\varphi(\sigma_i)$ is a binary random variable that is equal to $1$ with probability $p_\varphi$.
Since the sample signals are independent, the sum 
\begin{equation} \label{eq:K}
	K = \sum_{i \in [N]} \varphi (\sigma_{i})
\end{equation}
is a random variable following the binomial distribution $\mathrm{Binom} (N, p_\varphi)$, so the following approximation can be made
\begin{equation}
    \label{eq: p_phi approx}
    p_\varphi \approx \frac{K}{N}
\end{equation}
% satisfaction probability $p_\varphi$ can be approximated by the sample average $K/N$.

SMC aims to find a statistical assertion 
$\mathscr{A} \big( \sigma_1, \ldots, \sigma_N \big) \allowbreak \to \{H_\textrm{null}, H_\textrm{alt}\}$
that claims either $H_\textrm{null}$ or $H_\textrm{alt}$ holds based on the observed samples. Since $K$ is the sufficient statistics, the statistical assertion can be written as 
$$\mathscr{A} \big(K, N) \to \{H_\textrm{null}, H_\textrm{alt}\}.$$ 
Due to the randomness of $\sigma_1, \ldots, \sigma_N$, the value of $\mathscr{A}$ does not always agree with the truth value of $\mathbb{P}_{\sigma \sim \mathcal{S}} (\sigma \models \varphi) < p$. Thus, to capture these probabilistic errors, the false positive/false negative (FP/FN) ratios can be defined as
\begin{align} 
& \alpha_\textrm{FP} = \mathbb{P}_{\sigma_1, \ldots, \sigma_N \sim \mathcal{S}} \big( \mathscr{A} = H_\textrm{alt} \mid \mathbb{P}_{\sigma \sim \mathcal{S}} (\sigma \models \varphi) > p \big), \label{eq:fp_def}
\\ & \alpha_\textrm{FN} = \mathbb{P}_{\sigma_1, \ldots, \sigma_N \sim \mathcal{S}} \big( \mathscr{A} = H_\textrm{null} \mid \mathbb{P}_{\sigma \sim \mathcal{S}} (\sigma \models \varphi) \leq p \big). \label{eq:fn_def}
\end{align}
The FP ratio is the error probability of rejecting $H_\textrm{nullalt}$ when~\eqref{eq: SMC} holds and the FN ratio is the error probability of accepting $H_\textrm{null}$ when~\eqref{eq: SMC} does not hold.


The assertion $\mathscr{A}$ becomes more accurate, in terms of decreasing $\alpha_\textrm{FP}$ and $\alpha_\textrm{FN}$, when the number of samples $N$ increases. For any $N$, quantitative bounds of $\alpha_\textrm{FP}$ and $\alpha_\textrm{FN}$ can be derived by using either the confidence interval method~\cite{zarei2020statistical}, which only assumes $p_\varphi \neq p$, or the sequential probability ratio test method~\cite{sen2004statistical}, which requires a stronger assumption but is more efficient. This work focuses on the latter method since the following indifference parameter assumption holds in most applications, such as in~\cite{roohi2017statistical}.

\begin{assumption} \label{as:indifference}
There exists a known indifference parameter $\delta > 0$ such that $|p_\varphi - p| > \delta$ in~\eqref{eq: SMC}.
\end{assumption}

With Assumption~\ref{as:indifference}, we can consider two extreme cases in \eqref{eq: hypothesis testing}, according to~\cite{sen2004statistical},
\begin{align} \label{eq:problem 1 sht}
H_\textrm{null}: p_\varphi = p + \delta, \quad H_\textrm{alt}: p_\varphi = p - \delta.
\end{align}
To distinguish between $H_\textrm{null}$ or $H_\textrm{alt}$, we consider the likelihood ratio
\begin{equation} \label{eq:probability_ratio}
\lambda(K,N) = \frac{ (p+\delta)^{K} (1-p-\delta)^{N-K} }{ (p-\delta)^{K} (1-p+\delta)^{N-K} }.
\end{equation}
SMC aims to ensure $\alpha_\textrm{FP}, \alpha_\textrm{FN} \leq \alpha$ for a desired significance level $\alpha > 0$.
% \footnote{We choose the same threshold for $\alpha_\textrm{FP}$ and $\alpha_\textrm{FN}$ for simplicity. The method also applies to the case where two different thresholds for $\alpha_\textrm{FP}$ and $\alpha_\textrm{FN}$ are required (see~\cite{sen2004statistical}).}
Using sequential probability ratio tests~\cite{casella2002statistical}, SMC draws system samples until either condition on the right-hand-side of the following equation is satisfied before making a statistical assertion:
\begin{equation} \label{eq:sprt_test}
\mathscr{A} \big(K, N) = \begin{cases}
	H_\textrm{null}, &\text{ if } \lambda(K,N) \geq \frac{1 - \alpha}{\alpha}, \\
	H_\textrm{alt}, &\text{ if } \lambda(K,N) \leq \frac{\alpha}{1 - \alpha}.
\end{cases}
\end{equation}
As $N \to \infty$, by the binomial distribution, we have $\lambda(K,N) \to 0$ if $H_\textrm{null}$ holds or $\lambda(K,N) \to \infty$ if $H_\textrm{alt}$ holds, so \eqref{eq:sprt_test} stops with probability $1$.
% This procedure can be implemented incrementally by Algorithm~\ref{alg:1}.

% \begin{algorithm}[!t]

% \caption{Statistical model checking of $\mathbb{P}_{\sigma \sim \mathcal{S}} (\sigma \models \varphi) < p$.\label{alg:1}}

% \begin{algorithmic}[1]
% 	\Require Probabilistic model $\mathcal{S}$, desired significance level $\alpha$, and indifference parameter $\delta$.
	
% 	\State $N \gets 0$, $K \gets 0$, $\lambda \gets 1$.
	
% 	\While{True}
	
% 	\State Draw a new sample signal $\sigma$ from $\mathcal{S}$.
	
% 	\State $K \gets K + \varphi(\sigma)$, $N \gets N + 1$.
	
% 	\State $\lambda \gets \lambda \frac{ (p+\delta)^{\varphi(\sigma)} (1-p-\delta)^{1-\varphi(\sigma)} }{ (p-\delta)^{\varphi(\sigma)} (1-p+\delta)^{1-\varphi(\sigma)} }$ .
	
% 	\If {$\lambda \geq \frac{\alpha}{1 - \alpha}$} Return $H_\textrm{null}$
	
% 	\ElsIf {$\lambda \leq \frac{1 - \alpha}{\alpha}$} Return $H_\textrm{alt}$

% 	\Else \ Continue

% 	\EndIf 

% 	\EndWhile
	
% \end{algorithmic}
% \end{algorithm}

% \begin{remark} \label{rem:2}
% By Assumption~\ref{as:indifference}, we do not distinguish between checking $p_\varphi > p$ or checking $p_\varphi \geq p$ in~\eqref{eq: SMC}. In addition, by the semantics of STL in Section~\ref{sec:prelim}, checking $p_\varphi < p$ or $p_\varphi \leq p$ is equivalent to checking $p_{\neg \varphi} \geq 1 - p$ or $p_{\neg \varphi} > 1 - p$. Thus, the method for checking $p_\varphi > p$ applies to the other three cases.
% \end{remark}



% \section{Expected Differential Privacy for Statistical Model Checking}
% \label{sec:algorithm}
% In this section, we show that the termination time and output of Algorithm~\ref{alg:1} can be randomized, to achieve expected differential privacy. Our approach is based on a new sensitivity analysis and a novel exponential mechanism for randomizing the termination step.

\subsection{\my{Standard differential privacy and challenges}} \label{sub: sdp}
\todo{REPHRASE THIS SECTION}
\my{We denote the statistical model checking Algorithm~\ref{alg:1} by $\mathscr{A}$. The algorithm $\mathscr{A}$ is sequential: it samples signals $\sigma_1, \sigma_2, \ldots$ from the probabilistic model $\mathcal{S}$ until its termination condition is satisfied. Namely, it stops after a sampled data-dependent number of iterations $\tau_\mathscr{A} \in \nat$ and results in an output $o_\mathscr{A} $. With a slight abuse of notation, for an input sequence of sampled signals $\sigma_{1:\infty} = (\sigma_1, \sigma_2, \ldots)$, we write the termination step and output as functions of $\sigma_{1:\infty}$ by $\tau_\mathscr{A}  (\sigma_{1:\infty})$ and $o_\mathscr{A}  (\sigma_{1:\infty})$, respectively.}

\my{Differential privacy aims to prevent malicious inference on $\sigma_{1:\infty}$. Roughly, Algorithm $\mathscr{A}$ is differentially private if an attacker cannot infer the value of $\sigma_i$ even if they can observe $(\tau_\mathscr{A} (\sigma_{1:\infty}), o_\mathscr{A}  (\sigma_{1:\infty}))$ and the values of the rest of the entries $\sigma_{-i}$ of $\sigma_{1:\infty}$, for any sequence $\sigma_{1:\infty}$ and entry $\sigma_i$ in $\sigma_{1:\infty}$.~\cite{dwork2008differential}. Clearly, for a deterministic Algorithm $\mathscr{A}$, the value of $\sigma_i$ can be inferred when the inverse of $\tau_\mathscr{A} (\cdot)$ and $o_\mathscr{A} (\cdot)$ is unique after knowing the value of $\sigma_{-i}$.}

\my{A common approach to achieve differential privacy is to randomize Algorithm $\mathscr{A}$, such that even for the same input sequence $\sigma_{1:\infty}$, the algorithm is randomly executed in slightly different ways and yields different observations. For a randomized algorithm $\mathscr{B}$ of $\mathscr{A}$, although the randomization prevents the intruder to take the inverse of $\tau_{\mathscr{B}} (\cdot)$ and $o_{\mathscr{B}} (\cdot)$, the intruder can still infer the value of $\sigma_i$ by observing the difference in $\tau_{\mathscr{B}}  (\sigma_{1:\infty})$ and $o_{\mathscr{B}}  (\sigma_{1:\infty})$ when the value of $\sigma_{-i}$ is fixed and only the value of $\sigma_i$ changes. To measure the distance between two sequences, we recall the definition of Hamming distance. }

\my{Differential privacy requires a bound on the worst case change in the probabilities of the random observations for two adjacent input sequences. If the change in distribution is smaller, then it is harder for the intruder to infer the change in the input. We apply the standard notion of differential privacy in \cite{dwork2008differential} to Algorithm~\ref{alg:1} of Section~\ref{sec:prelim} in the following definition.}


\my{\begin{definition} \label{def:differential privacy}
A randomized sequential algorithm $\mathscr{B}$ is $\varepsilon$-differentially private, if it holds that
\begin{align} 
&\mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}), o_{\mathscr{B}} (\sigma_{1:\infty}) \big) \in \mathcal{O} \Big) \notag
\\ &\leq e^{\varepsilon} \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}'), o_\mathscr{A} (\sigma_{1:\infty}') \big) \in \mathcal{O} \Big) \label{eq:standard differential privacy}
\end{align}
for any two adjacent input sequences $\sigma_{1:\infty}$ and $\sigma_{1:\infty}'$ and any $\mathcal{O} \subseteq \mathbb{N} \times \{H_\textrm{null}, H_\textrm{alt}\}$. 
\end{definition}}

\my{The standard approach to make deterministic algorithms differentially private is to randomize their outputs by the exponential algorithm~\cite{mcsherry2007mechanism}. However, we show below that the exponential algorithm cannot achieve the differential privacy from Definition~\ref{def:differential privacy} for the statistical model checking method shown in Algorithm~\ref{alg:1}.}

\my{For simplicity, consider only the observation of the termination time $\tau_\mathscr{A} (\sigma_{1:\infty})$. We can define the sensitivity of termination time to changes in any single entry by 
\begin{equation}
\delta_{\tau_\mathscr{A}} := \max_{D_H (\sigma_{1:\infty}, \sigma_{1:\infty}') = 1} \big| \tau_\mathscr{A} (\sigma_{1:\infty}) - \tau_\mathscr{A} (\sigma_{1:\infty}') \big|,
\end{equation}
i.e., the maximal difference in termination time for any two adjacent input sequences of sample signals $\sigma_{1:\infty}$ and $\sigma_{1:\infty}'$.}

\my{If the sensitivity $\delta_{\tau_\mathscr{A}}$ is finite, then the following exponential algorithm achieves differential privacy. The exponential mechanism states that  randomizing algorithm $\mathscr{A}$ to $\mathscr{B}$ such that the probability of terminating at step $k$ is 
\begin{equation} \label{eq:exponential mechanism}
\mathbb{P}_{\mathscr{B}} (\tau_{\mathscr{B}} = k) = \frac{e^{- \varepsilon |\tau_\mathscr{A} - k| / \delta_{\tau_\mathscr{A}}}}{\sum_{h \in \mathcal{H}} e^{- \varepsilon |\tau_\mathscr{A} - h| / \delta_{\tau_\mathscr{A}}}},
\end{equation}
where $\mathcal{H} \subseteq \nat$ is the set of possible values of $\mathscr{A}$, and $\mathbb{P}_{\mathscr{B}}$ means that the randomness should come from the algorithm $\mathscr{B}$ itself. The exponential mechanism~\eqref{eq:exponential mechanism} is $2 \varepsilon$-differentially private~\cite{mcsherry2007mechanism}, since for any two adjacent $\sigma_{1:\infty}$ and $\sigma_{1:\infty}'$, it holds by the definition of sensitivity that for any $k \in \nat$,
\begin{equation} \label{eq:1}
\frac{e^{- \varepsilon  |\tau_\mathscr{A} (\sigma_{1:\infty}) - k| / \delta_{\tau_\mathscr{A}}}}{e^{- \varepsilon  |\tau_\mathscr{A} (\sigma_{1:\infty}') - k| / \delta_{\tau_\mathscr{A}}}} \leq e^{\varepsilon |\tau_\mathscr{A} (\sigma_{1:\infty}) - \tau_\mathscr{A} (\sigma_{1:\infty}')| / \delta_{\tau_\mathscr{A}}} \leq e^{\varepsilon},
\end{equation}
where the first inequality holds by applying the triangle inequality. Since~\eqref{eq:1} holds for any $k$, we have
\begin{equation} \label{eq:2}
\frac{\sum_{h \in \mathcal{H}} e^{- \varepsilon  |\tau_\mathscr{A} (\sigma_{1:\infty}) - h| / \delta_{\tau_\mathscr{A}}}}{\sum_{h \in \mathcal{H}} e^{- \varepsilon  |\tau_\mathscr{A} (\sigma_{1:\infty}') - h| / \delta_{\tau_\mathscr{A}}}} \leq e^\varepsilon.
\end{equation}
Thus, the probability ratio satisfies
\begin{equation} \label{eq:3}
\frac{\mathbb{P}_{\mathscr{B}} \big( \tau_{\mathscr{B}}(\sigma_{1:\infty}) = k \big)}{\mathbb{P}_{\mathscr{B}} \big( \tau_{\mathscr{B}}(\sigma_{1:\infty}') = k \big)} \leq e^{2 \varepsilon}.
\end{equation}}


\my{The above technique depends critically on the boundedness of the sensitivity $\delta_{\tau_\mathscr{A}}$, which is generally true for non-sequential algorithms~\cite{mcsherry2007mechanism}. However, this condition is violated for Algorithm~\ref{alg:1}, as shown in Example~\ref{ex:counter}.}

% To achieve EDP, the termination time and output of \eqref{eq:sprt_test} should be randomized. This will be done by carefully adding a randomization algorithm to the termination conditions.


\subsection{Analysis of termination time for statistical model checking} 
\label{sub:expected sensitivity analysis}

The sample termination time and the output $\big( \tau_\mathscr{A}, o_\mathscr{A} \big)$ of \eqref{eq:sprt_test} depend on the likelihood ratio $\lambda(N,K)$ in \eqref{eq:probability_ratio}. The log-likelihood ratio $\Lambda_N$ will be considered for analysis:
\begin{equation} \label{eq:llr}
\Lambda_N = \ln \lambda(K,N) = K s_+ - (N - K) s_-, \text{ where}
\end{equation}
$$
s_+ := \ln \frac{ p+\delta }{ p-\delta } > 0 \text{ and} \quad s_- := \ln \frac{ 1-p+\delta }{ 1-p-\delta } > 0
$$
% $$K = \sum_{i \in [N]} \varphi (\sigma_{i})$$ 
% is an random variable that follows the binomial distribution $\mathrm{Binom} (N, p_\varphi)$.

Using \eqref{eq: p_phi approx}, it can be seen that \eqref{eq:llr} forms an asymmetric random walk with probabilities and step sizes being $(p_\varphi, s_+)$ and $(1 - p_\varphi, -s_-)$.
% \begin{lemma} \label{lem:random walk}
% The log-likelihood ratio $\Lambda_N$ forms an asymmetric random walk with probabilities and step sizes being $(p_\varphi, s_+)$ and $(1 - p_\varphi, -s_-)$.
% \end{lemma}
% \begin{proof}
% By equation~\eqref{eq:llr}, we have $\Lambda_{0} = 0$ and 
% $$
% \Lambda_{N+1} = \begin{cases}
% \Lambda_{N} + s_+, & \text{ with probability } p_\varphi \\ 
% \Lambda_{N} - s_-, & \text{ with probability } 1 - p_\varphi. \\
% \end{cases}
% $$
% \end{proof}
% By Lemma~\ref{lem:random walk}
Thus, \eqref{eq:sprt_test} can be seen as a random walk that terminates at the following upper or lower bounds
\begin{align} \label{eq:stopping condition}
    B_+ := \ln \frac{1-\alpha}{\alpha} > 0, \quad B_- := - \ln \frac{1-\alpha}{\alpha} < 0
\end{align}
which will be modified with a randomization algorithm to ensure differential privacy.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Starting from here, this part is used in the "Expected sensitivity analysis for SMC"
% I don't think sensitivity analysis will be important here?
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% From Lemma~\ref{lem:random walk}, the average step size of the random walk $\Lambda_N$ is 
% % \hussein{ put $\mathcal{S}$ in the subscript of $\mathbb{E}$ ?}
% \begin{align}
% D := & \mathbb{E}_{\sigma_1} \Lambda_1 = p_\varphi s_+ - (1 - p_\varphi) s_- \notag
% \\ & = p_\varphi \ln \frac{ p+\delta }{ p-\delta } - (1 - p_\varphi) \ln \frac{ 1-p+\delta }{ 1-p-\delta } \label{eq:Lambda_1}
% \end{align} 
% When $B_+ \gg 1$ (equivalently, $B_- = - B_+ \ll -1$), we can prove that if $p_\varphi > p + \delta$, then the average step size is positive and the asymmetric random walk $\Lambda_N$ will hit the upper bound $B_+$ with probability $1 - \alpha$ and the lower bound $B_-$ with probability $\alpha$. Similarly, if $p_\varphi < p - \delta$, then the average step size is negative and the asymmetric random walk $\Lambda_N$ will hit the lower bound $B_-$ with probability $1 - \alpha$ and the upper bound $B_+$ with probability $\alpha$. 

% The average termination time $\tau_{\mathscr{A}} (\sigma_{1:\infty})$ satisfies the stopping time property of random processes~\cite{casella2002statistical}, i.e., 
% % \hussein{citation? subscripts for expectations?}
% \begin{align} 
% \mathbb{E}_{\sigma_{1:\infty}} [\Lambda_{\tau_{\mathscr{A}} (\sigma_{1:\infty})}] 
% & = \mathbb{E}_{\sigma_1} \Lambda_{1} \mathbb{E}_{\sigma_{1:\infty}} [ \tau_{\mathscr{A}} (\sigma_{1:\infty}) ] \notag
% \\ & = D \mathbb{E}_{\sigma_{1:\infty}} [ \tau_{\mathscr{A}} (\sigma_{1:\infty}) ]. \label{eq:stopping time property}
% \end{align}
% % by setting $\mathbb{E}_{\sigma_{1:\infty}} \Lambda_{\tau_{\mathscr{A}} (\sigma_{1:\infty})} 
% %  = B_+$ for $\mathbb{E}_{\sigma_1} \Lambda_{1} > 0$ and $ = B_-$ for $\mathbb{E}_{\sigma_1} \Lambda_{1} < 0$.
% % This equation shows the expected stopping position is equal to the expected step size multiplied by the termination time. Accordingly, the expected termination time is
% % \begin{align}
% % \mathbb{E} \tau_{\mathscr{A}} = \frac{\mathbb{E} \Lambda_{\tau_{\mathscr{A}}}}{\mathbb{E} \Lambda_{1}} & = \frac{(1 - 2 \alpha) \ln \frac{1-\alpha}{\alpha}}{\big| p_\varphi \ln \frac{ p+\delta }{ p-\delta } - (1 - p_\varphi) \ln \frac{ 1-p+\delta }{ 1-p-\delta } \big|} \notag
% % \\ & \approx \frac{\ln \frac{1-\alpha}{\alpha}}{\big| p_\varphi \ln \frac{ p+\delta }{ p-\delta } - (1 - p_\varphi) \ln \frac{ 1-p+\delta }{ 1-p-\delta } \big|} \label{eq:E tau}
% % \end{align}
% % for $\alpha \ll 1$. 



% \subsection*{Expected sensitivity analysis for statistical model checking}

% Now we define the sensitivity of the average termination time $\tau_\mathscr{A} (\sigma_{1:\infty})$ to single entry perturbations in the input sequence in the following equation: 
% \begin{equation} \label{eq:expected sensitivity}
% \Delta_{\tau_\mathscr{A}} := \max_{n \in \mathbb{N}, \sigma_n, \sigma'_n} \big| \mathbb{E}_{\sigma_{-n}} \tau_\mathscr{A} (\sigma_{1:\infty}) - \mathbb{E}_{\sigma_{-n}'} \tau_\mathscr{A} (\sigma_{1:\infty}') \big|,
% \end{equation}
% where $\sigma_{-n}$ and $\sigma_{-n}'$ are two random sequences of signals obeying the distribution of the probabilistic model $\mathcal{S}$. 
% We call $\Delta_{\tau_\mathscr{A}}$ the {\em expected sensitivity} of termination time. Expected sensitivity $\Delta_{\tau_\mathscr{A}}$ represents the maximal change in the average termination time over input sequences sampled from the probabilistic model $\mathcal{S}$ when arbitrarily changing the value of an arbitrary $n^{\mathit{th}}$ entry. %, assuming that the rest of the entries are randomly sampled from the probabilistic model $\mathcal{S}$. 

% For 
% %the statistical model checking algorithm $\mathscr{A}$
% Algorithm~\ref{alg:1}, we can use equation~\eqref{eq:stopping time property} to compute the expected sensitivity as shown in the following lemmas.

% \begin{lemma} \label{lem:termination time}
% For $D > 0$ in equation~\eqref{eq:Lambda_1}, 
% consider the random walk $\Lambda_N$ from Lemma~\ref{lem:random walk} for hitting any two absorbing bounds $A \gg \max\{s_+, s_-\}$ and $-B \ll - \max\{s_+, s_-\}$, the probability of hitting $B$ is $\approx e^{-B}$ and 
% the expected termination time is given by
% $$
% \mathbb{E}_{\sigma_{1:\infty}} [ \tau_{\mathscr{A}} (\sigma_{1:\infty}) ] \approx \frac{ A (1 - e^{-B})  - B e^{-B} }{D}.
% $$
% \end{lemma}

% \begin{proof}
% Let $a$ and $b$ be the probabilities of hitting the bounds $A$ and $B$ respectively. We have $a+b =1$, since the random walk terminates with probability $1$. For $D > 0$, when $A \gg \max\{s_+, s_-\}$ and $-B \ll - \max\{s_+, s_-\}$, we have from~\cite{casella2002statistical} that
% $$
% b \approx \frac{1 - e^{-A}}{e^{B}} \approx e^{-B}.
% $$
% The first approximate equality is due to the discrete steps in the random walk, which is negligible when $A \gg \max\{s_+, s_-\}$ and $-B \ll - \max\{s_+, s_-\}$.
% By the stopping time property~\eqref{eq:stopping time property}, we have the lemma holds.
% \end{proof}



% \begin{lemma} \label{lem:expected sensitivity}
% The expected sensitivity of the termination time $\tau_{\mathscr{A}}$ satisfies
% \begin{equation} \label{eq:Delta}
% \Delta_{\tau_\mathscr{A}} = \frac{s_+ + s_-}{|D|}
% = \frac{\ln \frac{ p+\delta }{ p-\delta } + \ln \frac{ 1-p+\delta }{ 1-p-\delta }}{\big| p_\varphi \ln \frac{ p+\delta }{ p-\delta } - (1 - p_\varphi) \ln \frac{ 1-p+\delta }{ 1-p-\delta } \big|},    
% \end{equation}
% where $s_+$ and $s_-$ are from equation~\eqref{eq:llr} and $D$ is from equation~\eqref{eq:Lambda_1}.
% \end{lemma}

% \begin{proof}
% Without loss of generality, consider the case of $D > 0$ in equation~\eqref{eq:Lambda_1}. The case of $D < 0$ can be proved similarly.
% Consider any two input sequences $\sigma_{1:\infty}$ and $\sigma_{1:\infty}'$ for Algorithm~\ref{alg:1}, where $\sigma_1$ and $\sigma_1'$ are chosen such that $\sigma_1 \models \varphi$ and $\sigma_1' \not\models \varphi$, and $\sigma_{2:\infty}$ and $\sigma_{2:\infty}'$ are drawn in an i.i.d. manner from the probabilistic model $\mathcal{S}$.
% Then, for the input sequence $\sigma_{1:\infty}$, the log-likelihood ratio $\Lambda_N$ follows a random walk that starts at $s_+$ after the first step. To derive the termination time to hit either $B_+$ or $B_-$ from equation~\eqref{eq:stopping condition}, we set $A := B_+ - s_+$ and $B := B_- - s_+$ in Lemma~\ref{lem:termination time} to obtain  
% % \todo{sometimes $\tau_\mathcal{A}$ is treated as a function of $\sigma$ and sometimes as a value, the notation should be unified in addition to the terminology. Also the expectations should have subscripts. Shouldn't $\Lambda_{1}$ be also a function of $\sigma$?}
% \begin{align*}
% & \mathbb{E}_{\sigma_{2:\infty}} [ \tau_{\mathscr{A}} (\sigma_{1:\infty}) ] 
% \\ & = 1 + \frac{(B_+ - s_+) (1 - e^{B_- - s_+}) + (B_- - s_+) e^{B_- - s_+} }{D}.
% \end{align*} 
% Similarly, by setting $A = B_+ + s_-$ and $B = B_- + s_-$ in Lemma~\ref{lem:termination time} as the bounds for the random walk of the log-likelihood ratio $\Lambda'_N$ of $\sigma'_{2:\infty}$, we have
% \begin{align*}
% & \mathbb{E}_{\sigma_{2:\infty}'} [ \tau_{\mathscr{A}} (\sigma_{1:\infty}') ] 
%  \\ & = 1 + \frac{(B_+ + s_-) (1 - e^{B_- + s_-}) + (B_- + s_-) e^{B_- + s_-} }{D}.
% \end{align*}
% Considering $s_+, -s_- \ll B_+, -B_-$, the subtraction of the two equations shown above gives
% \begin{align*}
% \mathbb{E}_{\sigma_{2:\infty}} \tau_{\mathscr{A}} (\sigma_{1:\infty}) - \mathbb{E}_{\sigma_{2:\infty}'} \tau_{\mathscr{A}} (\sigma_{1:\infty}') \approx \frac{s_+ + s_-}{D},
% \end{align*}
% considering that $e^{B_-} \ll 1$. This proves the bound of expected sensitivity~\eqref{eq:expected sensitivity} stated in the lemma for alternating the first entry. The case of other entries can be proved similarly.
% \end{proof}





% When the expected sensitivity $\Delta_{\tau_\mathscr{A}} < \infty$ is finite, we can apply a modified version of the exponential mechanism described in Section~\ref{sub:Laplace} to Algorithm~\ref{alg:1} to achieve expected differential privacy for the termination time. This is shown in the following lemma. 


% \begin{lemma} \label{lem:exponential mechanism 2}
% For a sequential algorithm $\mathscr{A}$ with a deterministic termination time $\tau_\mathscr{A}$, consider another sequential algorithm $\mathscr{B}$ with the same input and output spaces as $\mathscr{A}$ but with a random termination time $\tau_{\mathscr{B}}$ that satisfies 
% \begin{align} 
% & \mathbb{P}_{\mathscr{B}} \big( \mathbb{E}_{\sigma_{1:\infty}} \big[ \tau_\mathscr{B} (\sigma_{1:\infty})\big] = k \big) \notag
% \\ &  
% \qquad = \frac{e^{- \varepsilon |k - \mathbb{E}_{\sigma_{1:\infty}} [\tau_\mathscr{A} (\sigma_{1:\infty})]| / \Delta_{\tau_\mathscr{A}}}}{\sum_{h \in \nat} e^{- \varepsilon |h - \mathbb{E}_{\sigma_{1:\infty}} [\tau_\mathscr{A} (\sigma_{1:\infty})]| / \Delta_{\tau_\mathscr{A}}}}, \label{eq:exponential mechanism 2}
% \end{align}
% where $\sigma_{1:\infty}$ is a random sequence of signals obeying the distribution of the probabilistic model $\mathcal{S}$. 
% Then, it is  $\varepsilon$-expectedly differentially private in termination time.
% \end{lemma}


% \begin{proof}
% Without loss of generality, assuming $D > 0$ in equation~\eqref{eq:Lambda_1}, we will prove the condition~\eqref{eq:edp termination time} of Definition~\ref{def:expected differential privacy} for $n = 1$, i.e.,
% \begin{align}
% \frac{\mathbb{P}_{\mathscr{B}} \big( \mathbb{E}_{\sigma_{2:\infty}} \big[ \tau_\mathscr{B} (\sigma_{1:\infty}) ] = k \big)}{\mathbb{P}_{\mathscr{B}} \big( \mathbb{E}_{\sigma_{2:\infty}'} \big[ \tau_\mathscr{B} (\sigma_{1:\infty}') ] = k )} \leq e^{2 \varepsilon}, \label{eq:to prove}
% \end{align}
% for any pair of signals $\sigma_1$ and $\sigma'_1$, 
% where $\sigma_{2:\infty}$ and $\sigma_{2:\infty}'$ are random sequences of i.i.d. signals obeying the distribution of the probabilistic model $\mathcal{S}$. For simplicity, we consider the case of $\varphi(\sigma_1) = 1$ and $\varphi(\sigma_1') = 0$. The case of $\varphi(\sigma_1) = 0$ and $\varphi(\sigma_1') = 1$ can be handled similarly. The cases of $\varphi(\sigma_1) = \varphi(\sigma_1') = 0$ and $\varphi(\sigma_1) = \varphi(\sigma_1') = 1$ are trivial. 


% When $\varphi(\sigma_1) = 1$, by the stopping time property~\eqref{eq:stopping time property}, we have 
% \begin{align*}
% & \mathbb{P}_{\mathscr{B}} \big( \mathbb{E}_{\sigma_{2:\infty}} \big[ \tau_\mathscr{B} (\sigma_{1:\infty}) ] = k \big)
%  \\ & = \mathbb{P}_{\mathscr{B}} \big( \mathbb{E}_{\sigma_{2:\infty}} \big[ \tau_\mathscr{B} (\sigma_{2:\infty}) ] = k - \frac{s_+}{D} \big)
% \end{align*}
% where $s_+$ is given by equation \eqref{eq:llr} with $\mathbb{E}_{\sigma_{2:\infty}} \Lambda_{\tau_{\mathscr{B}} (\sigma_{1:\infty})} - \mathbb{E}_{\sigma_{2:\infty}} \Lambda_{\tau_{\mathscr{B}} (\sigma_{2:\infty})} = s_+$.
% % $$
% % s_+ = \mathbb{E}_{\sigma_{1:\infty}} [\Lambda_{\tau_{\mathscr{A}} (\sigma_{1:\infty})}] - \mathbb{E}_{\sigma_{2:\infty}} [\Lambda_{\tau_{\mathscr{A}} (\sigma_{2:\infty})}] = D \mathbb{E}_{\sigma_{1:\infty}} [ \tau_{\mathscr{A}} (\sigma_{1:\infty}) ] - D \mathbb{E}_{\sigma_{2:\infty}} [ \tau_{\mathscr{A}} (\sigma_{2:\infty}) ].
% % $$


% By viewing $\sigma_{2:\infty}$ as a new random walk, we can apply equation \eqref{eq:exponential mechanism 2} and derive
% \begin{align}
% & \mathbb{P}_{\mathscr{B}} \big( \mathbb{E}_{\sigma_{2:\infty}} \big[ \tau_\mathscr{B} (\sigma_{2:\infty}) ] = k - \frac{s_+}{D} \big) \notag
% \\ & = \mathbb{P}_{\mathscr{B}} \big( \mathbb{E}_{\sigma_{1:\infty}} \big[ \tau_\mathscr{B} (\sigma_{1:\infty}) ] = k - \frac{s_+}{D} + 1 \big) \notag
% \\ & = \frac{e^{- \varepsilon |k - \frac{s_+}{D} + 1 - \mathbb{E}_{\sigma_{1:\infty}} [\tau_\mathscr{A} (\sigma_{1:\infty})]| / \Delta_{\tau_\mathscr{A}}}}{\sum_{h \in \nat} e^{- \varepsilon |h - \frac{s_+}{D} + 1 - \mathbb{E}_{\sigma_{1:\infty}} [\tau_\mathscr{A} (\sigma_{1:\infty})]| / \Delta_{\tau_\mathscr{A}}}} \label{eq:tau sigma}
% \end{align}
% Similarly, we have 
% \begin{align}
% & \mathbb{P}_{\mathscr{B}} \big( \mathbb{E}_{\sigma_{2:\infty}'} \big[ \tau_\mathscr{B} (\sigma_{1:\infty}') ] = k \big) \notag
% \\ & = \frac{e^{- \varepsilon |k + \frac{s_-}{D} + 1 - \mathbb{E}_{\sigma_{1:\infty}'} [\tau_\mathscr{A} (\sigma_{1:\infty}')]| / \Delta_{\tau_\mathscr{A}}}}{\sum_{h \in \nat} e^{- \varepsilon |h + \frac{s_-}{D} + 1 - \mathbb{E}_{\sigma_{1:\infty}'} [\tau_\mathscr{A} (\sigma_{1:\infty}')]| / \Delta_{\tau_\mathscr{A}}}} \label{eq:tau sigma'}
% \end{align}


% % Other cases can be proved similarly. From equation~\eqref{eq:exponential mechanism 2}, we have
% % $$ 
% % \big| \mathbb{E}_{\sigma_{-n}} [\tau_\mathscr{A} (\sigma_{1:\infty})] - \mathbb{E}_{\sigma_{-n}'} [\tau_\mathscr{A} (\sigma_{1:\infty}')] \big| \leq \Delta_{\tau_\mathscr{A}},
% % $$
% % Since the above inequality holds for any $\sigma_n$ and $\sigma'_n$, 
% % taking the expected values of $\sigma_n$ and $\sigma'_n$ on both sides and applying Jensen's inequality gives
% % $$ 
% % \big| \mathbb{E}_{\sigma_{1:\infty}} [\tau_\mathscr{A} (\sigma_{1:\infty})] - \mathbb{E}_{\sigma_{1:\infty}'} [\tau_\mathscr{A} (\sigma_{1:\infty}')] \big| \leq \Delta_{\tau_\mathscr{A}}.
% % $$

% By the triangular inequality and using the definition of $\Delta_{\tau_\mathscr{A}}$ from~\eqref{eq:Delta}, the ratio of the numerators of equations \eqref{eq:tau sigma} and \eqref{eq:tau sigma'} satisfies
% \begin{equation} \label{eq:4}
% e^{-\varepsilon} \leq \frac{e^{- \varepsilon |k - \frac{s_+}{D} + 1 - \mathbb{E}_{\sigma_{1:\infty}} [\tau_\mathscr{A} (\sigma_{1:\infty})]| / \Delta_{\tau_\mathscr{A}}}}{e^{- \varepsilon |k + \frac{s_-}{D} + 1 - \mathbb{E}_{\sigma_{1:\infty}'} [\tau_\mathscr{A} (\sigma_{1:\infty}')]| / \Delta_{\tau_\mathscr{A}}}} \leq e^\varepsilon.
% \end{equation}
% Since~\eqref{eq:4} holds for any $k$, we have
% \begin{equation} \label{eq:5}
% e^{-\varepsilon} \leq \frac{\sum_{h} e^{- \varepsilon |h - \frac{s_+}{D} + 1 - \mathbb{E}_{\sigma_{1:\infty}} [\tau_\mathscr{A} (\sigma_{1:\infty})]| / \Delta_{\tau_\mathscr{A}}}}{\sum_{h} e^{- \varepsilon |h + \frac{s_-}{D} + 1 - \mathbb{E}_{\sigma_{1:\infty}'} [\tau_\mathscr{A} (\sigma_{1:\infty}')]| / \Delta_{\tau_\mathscr{A}}}} \leq e^\varepsilon.
% \end{equation}
% Thus, by taking the ratios of~\eqref{eq:4} and~\eqref{eq:5} and applying \eqref{eq:tau sigma} and \eqref{eq:tau sigma'} results in that for any $k \in \mathbb{N}$, we can derive~\eqref{eq:to prove}.

%  The condition~\eqref{eq:edp termination time} of Definition~\ref{def:expected differential privacy} for $n \neq 1$ can be proved similarly.
% \end{proof}





\subsection{Causal randomization for differential privacy of termination time}
\label{sub:randomizing the algorithm}

With the upper and lower bounds of the random walk identified, this work seeks to add a causal randomization mechanism to the sample termination time of \eqref{eq:sprt_test}.
% Algorithm~\ref{alg:1} that achieves the probability distribution in equation~\eqref{lem:exponential mechanism 2}.


\my{(This is the only paragraph I couldn't understand.)} A trivial addition of random noise to the deterministic termination time is not causal. % Consider the implementation of the randomization mechanism.
If the deterministic termination time plus the random noise is $n \leq k = \tau_{\mathscr{A}} (\sigma_{1:\infty})$, the randomized algorithm can draw additional $n - \tau_{\mathscr{A}}$ samples and ignore their values. However, if $n < k = \tau_{\mathscr{A}} (\sigma_{1:\infty})$, then the randomized algorithm $\mathscr{B}$ will not be able to causally predict that it should stop before reaching the deterministic termination time of $\mathscr{A}$. %  cannot be done causally in time. 
% there is no way the randomized algorithm can reverse the sampling
% This shows the difficulty in directly randomizing the termination time of Algorithm~\ref{alg:1} to achieve expected differential privacy. 

% Our solution is to 
Instead, the sample termination time of \eqref{eq:sprt_test} can be randomized by modifying the upper and lower bounds as follows
% Recall from equation~\eqref{eq:stopping condition} that Algorithm~\ref{alg:1} stops upon reaching the upper or lower bounds $B_+$ and $B_-$, respectively. We modify these bounds as follows:
\begin{align} \label{eq:randomized stopping condition}
& B_+ = \ln \frac{1-\alpha}{\alpha} + L \text{ and} \quad B_- = - \ln \frac{1-\alpha}{\alpha} - L, \text{ where }  \notag 
\\ & L \sim \textrm{Exp} \bigg( \frac{\varepsilon}{\ln \frac{ p+\delta }{ p-\delta } + \ln \frac{ 1-p+\delta }{ 1-p-\delta }} \bigg),
\end{align}
which is shown in Algorithm~\ref{alg:2}.
% The modified version of Algorithm~\ref{alg:1} is shown in Algorithm~\ref{alg:2}.
% \hussein{that achieves} expected differential privacy. 
% \todo{You're using a different definition of $L$ in Algorithm 2 than the one in (29).}


% \todo{Also, shouldn't this be a geometric distribution instead? Shouldn't L be an integer?}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The following lemmas depend on the expected sensitivity analysis in order to make sense. Since the expected sensitivity section was commented out, this section shall also be commented out.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{lemma} \label{lem:random bounds}
% The termination time of Algorithm~\ref{alg:2} satisfies the distribution shown in equation~\eqref{eq:exponential mechanism 2}.
% \end{lemma}

% \begin{proof}
% We denote Algorithm~\ref{alg:2} by ${\mathscr{B}}$ and let $B = \ln \frac{1-\alpha}{\alpha}$. Without loss of generality, suppose that the average step size $D$ from~\eqref{eq:Lambda_1} of the random walk $\Lambda_N$ is $> 0$ . Following the randomized stopping  condition in equation~\eqref{eq:randomized stopping condition}, we have that for any $k \in \mathbb{N}$,
% \begin{align*} 
% & \mathbb{P}_L \big( \mathbb{E}_{\sigma_{1:\infty}} \big[ \tau_{\mathscr{B}} (\sigma_{1:\infty}) \big] = k \big)
% \\ & = \mathbb{P}_L \big( \mathbb{E}_{\sigma_{1:\infty}} \big[ \Lambda_k (\sigma_{1:\infty}) \big] \geq B + L 
% \\ & \qquad \text{ and } \mathbb{E}_{\sigma_{1:\infty}} \big[ \Lambda_{k - 1} (\sigma_{1:\infty}) \big] < B + L \big)
% \\ & \text{[as $\mathbb{E}_{\sigma_{-n}} \big[ \Lambda_k (\sigma_{1:\infty}) \big]$ is increasing in $k$ when $D > 0$]}
% \\ & = \mathbb{P}_L \big( k D \geq B + L \text{ and } (k-1) D < B + L \big)
% \\ & \text{[using the stopping time property in equation~\eqref{eq:stopping time property}]}
% \\ & = \int_{(k-1) D - B}^{k D - B}
% \frac{\varepsilon}{\ln \frac{ p+\delta }{ p-\delta } + \ln \frac{ 1-p+\delta }{ 1-p-\delta }} e^{\frac{\varepsilon x}{\ln \frac{ p+\delta }{ p-\delta } + \ln \frac{ 1-p+\delta }{ 1-p-\delta }}} \d x
% \\ & \text{[using equation~\eqref{eq:randomized stopping condition}]}
% \\ & \approx \frac{D \varepsilon}{\ln \frac{ p+\delta }{ p-\delta } + \ln \frac{ 1-p+\delta }{ 1-p-\delta }} e^{\frac{\varepsilon (k D - B)}{\ln \frac{ p+\delta }{ p-\delta } + \ln \frac{ 1-p+\delta }{ 1-p-\delta }}} \propto e^{\frac{\varepsilon (k - B/D) }{\Delta_{\tau_\mathscr{A}}}} 
% \\ & \text{[using $D \ll B$ and~\eqref{eq:Delta}]}
% \end{align*}
% This leads to~\eqref{eq:exponential mechanism 2} since $\mathbb{E}_{\sigma_{1:\infty}} [\tau_\mathscr{A} (\sigma_{1:\infty})] \approx B/D$ from Lemma~\ref{lem:termination time}.
% \end{proof}

% Following the same process, we can apply the expected sensitivity analysis for $o_\mathscr{A}$ for Algorithm~\ref{alg:1}. 

% \begin{lemma} \label{lem:obs}
% The expected sensitivity $\Delta_{o_\mathscr{A}}$ of the output $o_{\mathscr{A}}$ of Algorithm~\ref{alg:1} is $\approx 0$, where $\Delta_{o_\mathscr{A}}$ is defined as 
% \begin{align}
% \Delta_{o_\mathscr{A}} & := \max_{n \in \mathbb{N}, \sigma_n, \sigma'_n} \big| \mathbb{E}_{\sigma_{-n}} o_\mathscr{A} (\sigma_{1:\infty}) - \mathbb{E}_{\sigma_{-n}'} o_\mathscr{A} (\sigma_{1:\infty}') \big|, \label{eq:expected sensitivity of output}
% \end{align}
% and $\sigma_{-n}$ and $\sigma_{-n}'$ are random sequences of i.i.d. signals obeying the distribution of the probabilistic model $\mathcal{S}$.
% \end{lemma}

% \begin{proof}
% Consider $n = 1$. For $D > 0$, Algorithm~\ref{alg:1} returns $0$ by hitting the bound $-B$ and returns $1$ by hitting the bound $B$, as defined in Definition~\ref{def:expected differential privacy}. By Lemma~\ref{lem:termination time}, when $\sigma_1 \models \varphi$, we have $\mathbb{P}_{\sigma_{2:\infty}} [o_\mathscr{A} (\sigma_{1:\infty}) = 0] = e^{-B+s_+}$ by viewing the log-likelihood ratio $\Lambda_N$ in Algorithm~\ref{alg:1} as a random walk starting from $s_+$ after the first step, instead of starting from zero in the first step. Similarly, when $\sigma_1 \not\models \varphi$, we have $\mathbb{P}_{\sigma_{2:\infty}} [o_\mathscr{A} (\sigma_{1:\infty}) = 0] = e^{-B-s_-}$. Thus, we have
% \begin{align}
% \Delta_{o_\mathscr{A}} & = \max_{\sigma_1, \sigma'_1} \big| \mathbb{E}_{\sigma_{2:\infty}} [o_\mathscr{A} (\sigma_{1:\infty})] - \mathbb{E}_{\sigma_{2:\infty}'} [o_\mathscr{A} (\sigma_{1:\infty}')] \big| \notag
% \\ & \leq | e^{-B+s_+} - e^{-B-s_-} | \approx 0.
% \end{align}
% The same analysis holds for $n \neq 1$.
% \end{proof}

% Thus, changing an arbitrary $n^{\mathit{th}}$ sample has almost no influence on the output of algorithm $\mathscr{A}$ in the expected sense. In sum, we present the following theorems.

With the modification, Algorithm~\ref{alg:2} is $2 \varepsilon$-expectedly differentially private
% \begin{theorem}
% Algorithm~\ref{alg:2} is $2 \varepsilon$-expectedly differentially private.
% \end{theorem}
% \begin{proof}
% It directly follows from Lemmas~\ref{lem:random bounds} and~\ref{lem:obs}.
% \end{proof}
and has a significance level less than $\alpha$.
% In addition to privacy, we provide the following results for the significance level of Algorithm~\ref{alg:2}.
% Furthermore, the causal randomization for differential privacy of termination time can potentially be applied to SMC of hyperproperties, which also uses the sequential probability ratio test to infer the truth value of formulas \cite{wang2021statistical}.
% \begin{theorem}
% Algorithm~\ref{alg:2} has a significance level (i.e., the upper bound on the probability that this algorithm returns a wrong answer) is less than $\alpha$.
% \end{theorem}

% \begin{proof}
% In Algorithm~\ref{alg:2}, the hitting bounds $B+L$ and $-B-L$ are always expanded versions of those of Algorithm~\ref{alg:1} since $L \geq 0$. Hence, the accuracy is improving because of drawing more samples. Specifically, following the standard analysis of sequential hypotheses testing~\cite{casella2002statistical}, for any value of $L$ in Algorithm~\ref{alg:2}, the significance level $\alpha_L$ for hitting the bounds $B+L$ and $-B-L$ satisfies 
% \begin{align*}
% \frac{1 - \alpha_L}{\alpha_L} = \ln B_+ \leq  \ln \frac{1-\alpha}{\alpha}
% \end{align*}
% since $L \geq 0$ in~\eqref{eq:randomized stopping condition}.
% This implies $\alpha_L \leq \alpha$ for any value of $L$. Thus, the theorem holds.
% \end{proof}

\begin{algorithm}[t]
\caption{Statistical model checking of $\mathbb{P}_{\sigma \sim \mathcal{S}} (\sigma \models \varphi) < p$ with expected differential privacy.\label{alg:2}}

\begin{algorithmic}[1]
\Require Probabilistic model $\mathcal{S}$, desired significance level $\alpha$, and indifference parameter $\delta$, privacy level $\varepsilon$.

\State $N \gets 0$, $K \gets 0$.

\State Log-likelihood ratio $\Lambda \gets 0$.

\State $B \gets \ln \frac{1-\alpha}{\alpha}$, $L \sim \textrm{Exp} \Big( \frac{\varepsilon}{\ln \frac{ p+\delta }{ p-\delta } + \ln \frac{ 1-p+\delta }{ 1-p-\delta }} \Big)$

\While{True}

\State Draw a sample signal $\sigma$ from $\mathcal{S}$.

\State $K \gets K + \varphi(\sigma)$, $N \gets N + 1$.

\State $\Lambda \gets \Lambda + \ln \frac{ (p+\delta)^{\varphi(\sigma)} (1-p-\delta)^{1-\varphi(\sigma)} }{ (p-\delta)^{\varphi(\sigma)} (1-p+\delta)^{1-\varphi(\sigma)} }$ .

\If {$\Lambda \geq B + L$} 

\State Return $H_\textrm{null}$ 

\ElsIf {$\Lambda \leq -B - L$} 

\State Return $H_\textrm{alt}$

\Else \ Continue

\EndIf 

\EndWhile

\end{algorithmic}
\end{algorithm}

% Finally, the causal randomization for differential privacy of termination time can potentially be applied to the statistical model checking of hyperproperties, which also uses the sequential probability ratio test to infer the truth value of formulas \cite{wang2021statistical}.

==> prelim.tex <==
\section{Preliminaries on Statistical Model Checking} \label{sec:prelim}

Real-world cyber-physical systems are typically subject to uncertainty in their parameters from different sources, e.g., thermal fluctuations in sensors/actuators. The probabilistic uncertainty is expressible by random variables drawn from probabilistic distributions, which may be unknown. For example, the uncertainty in the sensor readings can be expressed by the addition of a random noise. Such uncertainties can be captured by a probabilistic model. A key problem for the probabilistic model is whether a specification holds on a random system path with probability above some given threshold. Such a problem can be solved with provable probabilistic guarantees by statistical model checking. Below, we summarize previous work on statistical model checking algorithms based on sequentially probability ratio tests~\cite{legay2010statistical,agha2018survey}.


Consider a random signal (e.g., paths/trajectories) $\sigma$ from a probabilistic model $\mathcal{S}$. 
The model $\mathcal{S}$ can be either known or unknown and of general form (e.g., discrete, continuous, or hybrid).
% \todo{should we define probabilistic systems more formally?}
The goal of statistical model checking is to check the satisfaction probability of a specification $\varphi$. To start with, we check whether the probability of $\sigma$ satisfying $\varphi$ is greater than some given probability threshold $p \in [0,1]$, i.e.,
\begin{equation} \label{eq:problem 1}
	\mathbb{P}_{\sigma \sim \mathcal{S}} ( \sigma \models \varphi ) = p_\varphi > p,
\end{equation}
where $\models$ means ``to satisfy'' and $p_\varphi$ is the satisfaction probability of $\varphi$ on $\mathcal{S}$. 


Formally, the specifications are typically expressed by signal temporal logic (STL)~\cite{maler2004monitoring}, which contains a simple set of syntactic rules to describe the change of real-valued system variables in continuous time.
\my{I don't think we need an entire section on signal temporal logic so I commented it out.}
% The syntax of STL specifications is defined recursively by:
% \[
% \varphi :=
% f (\sigma) \geq 0
% \mid \neg \varphi
% \mid \varphi \land \varphi
% \mid \varphi \ \mathcal{U}_{[t_1,t_2]} \ \varphi,
% \]
% where $\sigma: \nnreal \to \real^n$ is a signal (i.e., a vector of real-valued system variables that changes over time), $f: \real^n \to \real$ is a real-valued function of the signal, and $[t_1, t_2]$ is a time interval with $t_2 > t_1 \geq 0$. Strictly speaking, $t_1$ and $t_2$ should be rational-valued or infinity. By recursively applying these syntactic rules, we can write arbitrarily complex STL specifications to express general specifications of interest.


% Given any STL specification $\varphi$, we can define whether a signal $\sigma$ satisfies it or not, written as $\sigma \models \varphi$ or $\sigma \not\models \varphi$, using the following semantic rules: 
% \begin{align*}
% & \sigma \models f (\sigma) \geq 0  & \ \Leftrightarrow \ &   f(\sigma(0)) \geq 0 \\
% & \sigma \models \neg \varphi  & \ \Leftrightarrow \ &  \sigma \not\models \varphi \\
% & \sigma \models \varphi \land \psi  & \ \Leftrightarrow \ &  \sigma \models \varphi \land \sigma \models \psi \\
% & \sigma \models \varphi \ \mathcal{U}_{[t_1,t_2]} \ \psi & \ \Leftrightarrow \ &  \exists t \in [t_1, t_2] \text{ such that } \sigma^{(t)} \models \psi \\
% & & & \land \forall t' < t, \sigma^{(t')} \models \varphi
% \end{align*}
% where $\sigma^{(t)}$ denotes the $t$-shift of $\sigma$, defined by $\sigma^{(t)}(t') = \sigma(t + t')$ for any $t' \in \nnreal$. 
% The first rule means that $\sigma$ satisfies $f (\sigma) \geq 0$ if and only if the initial value of $\sigma$ at time $t=0$ satisfies $f (\sigma(0)) \geq 0$. The fourth rule defined the ``until'' temporal operator; it means that $\sigma$ satisfies $\varphi \ \mathcal{U}_{[t_1,t_2]} \ \psi$ if and only if $\sigma$ satisfies $\varphi$ at all time instants before $t$ until it satisfies $\psi$ exactly at time $t$ for some $t \in [t_1,t_2]$. 

% Using the STL syntax and semantics, we can define other temporal operators such as ``finally'' (or ``eventually'') and ``always'', written as $\Diamond$ and $\square$. Specifically, 
% $\Diamond_{[t_1,t_2]} \varphi = \mathtt{True} \ \mathcal{U}_{[t_1,t_2]} \ \varphi$ 
% means the property $\varphi$ finally holds; and 
% $\square_{[t_1,t_2]} \varphi = \neg (\Diamond_{[t_1,t_2]} \neg\varphi)$ 
% means the property $\varphi$ always holds. In addition, although only the inequality symbol ``$>$'' is included in the STL syntax, we can express other inequalities symbols via the semantics. For example, $f (\sigma) > 0$ can be expressed by $ \neg \big( {-} f (\sigma) \geq 0 \big)$. Below, we will also use these operators or symbols in STL specifications.   

% \begin{example} \label{ex:1}
% Suppose $\sigma = (\sigma_1, \sigma_2)$ where $\sigma_1$ and $\sigma_2$ are the velocity and battery level of an electric vehicle. Then the specification
% $$(\sigma_1 > 5) \ \mathcal{U}_{[0, 10]} \ (\sigma_2 < 0.2)$$
% means the car velocity should be greater than $5$ before the battery level drops below $0.2$ within $10$ time units. 
% \end{example}




\subsection*{Sequential probability ratio test}

Statistical model checking handles the statement~\eqref{eq:problem 1} by formulating it as a hypothesis testing problem
\begin{align} \label{eq:problem 1 ht}
H_\textrm{null}: p_\varphi > p, \quad
H_\textrm{alt}: p_\varphi \leq p, 
\end{align}
where $H_\textrm{null}$ and $H_\textrm{alt}$ are the null and alternative hypotheses. Then, it infers whether $H_\textrm{null}$ or $H_\textrm{alt}$ holds by drawing sample signals $\sigma_1, \sigma_2, \ldots$ from the probabilistic model $\mathcal{S}$. As with previous work~\cite{legay2010statistical,agha2018survey}, we focus on samples that are drawn independently. 

\begin{remark} \label{rem:independent}
It has been shown that correlated samples can improve the efficiency of statistical model checking~\cite{wang2018statisticala,wang2019statistical}. However,  using correlated samples requires at least partial knowledge of the system dynamics to implement. On the other hand, independent sampling can apply to general black-box systems.
\end{remark}

The statistical model checking algorithm examines the correctness of $\varphi$ on each sample signals $\sigma_i$. This process can be performed automatically by existing model checking algorithms from~\cite{maler2004monitoring,roohi2018revisiting}. With a slight abuse of notation, we represent ``True'' and ``False'' by $1$ and $0$ and define the truth values by
\begin{equation} \label{eq:varphi}
\varphi(\sigma_i) = \begin{cases}
1, & \sigma_i \models \phi, \\
0, &\text{ otherwise.}
\end{cases}
\end{equation}
Each $\varphi(\sigma_i)$ is a binary random variable that is equal to $1$ with probability $p_\varphi$. Since the sample signals are independent, the sum 
\begin{equation} \label{eq:K}
	K = \sum_{i \in [N]} \varphi (\sigma_{i})
\end{equation}
is a random variable following the binomial distribution $\mathrm{Binom} (N, p_\varphi)$. Thus, the satisfaction probability $p_\varphi$ can be approximated by the sample average $K/N$.

Our goal is to find a statistical assertion 
$\mathscr{A} \big( \sigma_1, \ldots, \sigma_N \big) \allowbreak \to \{H_\textrm{null}, H_\textrm{alt}\}$
that claims either $H_\textrm{null}$ or $H_\textrm{alt}$ holds based on the observed samples. Moreover, since $K$ is the sufficient statistics, the statistical assertion can be written as 
$$\mathscr{A} \big(K, N) \to \{H_\textrm{null}, H_\textrm{alt}\}.$$ 
Due to the randomness of $\sigma_1, \ldots, \sigma_N$, the value of the statistical assertion $\mathscr{A}$ does not always agree with the truth value of $\mathbb{P}_{\sigma \sim \mathcal{S}} (\sigma \models \varphi) < p$. To capture these probabilistic errors, we define the false positive/false negative (FP/FN) ratios as
\begin{align} 
& \alpha_\textrm{FP} = \mathbb{P}_{\sigma_1, \ldots, \sigma_N \sim \mathcal{S}} \big( \mathscr{A} = H_\textrm{alt} \mid \mathbb{P}_{\sigma \sim \mathcal{S}} (\sigma \models \varphi) > p \big), \label{eq:fp_def}
\\ & \alpha_\textrm{FN} = \mathbb{P}_{\sigma_1, \ldots, \sigma_N \sim \mathcal{S}} \big( \mathscr{A} = H_\textrm{null} \mid \mathbb{P}_{\sigma \sim \mathcal{S}} (\sigma \models \varphi) \leq p \big). \label{eq:fn_def}
\end{align}
The FP ratio is the error probability of mistakenly rejecting the null hypotheses $H_\textrm{alt}$ while~\eqref{eq:problem 1} holds. The FN ratio is the error probability of mistakenly accepting the null hypotheses $H_\textrm{null}$ while~\eqref{eq:problem 1} does not hold.


Intuitively, the assertion $\mathscr{A}$ becomes more accurate in terms of decreasing $\alpha_\textrm{FP}$ and $\alpha_\textrm{FN}$ when the number of samples $N$ increases. For any $N$, quantitative bounds of $\alpha_\textrm{FP}$ and $\alpha_\textrm{FN}$ can be derived by using either the confidence interval method~\cite{zarei2020statistical} or the sequential probability ratio test method~\cite{sen2004statistical}. The former only assumes that $p_\varphi \neq p$. The latter requires the following stronger assumption but is more efficient. This work focuses on the latter method since the indifference parameter assumption holds in most applications (e.g., in~\cite{roohi2017statistical}).

\begin{assumption} \label{as:indifference}
There exists a known indifference parameter $\delta > 0$ such that $|p_\varphi - p| > \delta$ in~\eqref{eq:problem 1}.
\end{assumption}

With Assumption~\ref{as:indifference}, it suffices to consider the two extreme cases in hypothesis~\eqref{eq:problem 1 ht} according to~\cite{sen2004statistical}, i.e.,
\begin{align} \label{eq:problem 1 sht}
H_\textrm{null}: p_\varphi = p + \delta, \quad H_\textrm{alt}: p_\varphi = p - \delta.
\end{align}
To distinguish between $H_\textrm{null}$ or $H_\textrm{alt}$, we consider the likelihood ratio
\begin{equation} \label{eq:probability_ratio}
\lambda(K,N) = \frac{ (p+\delta)^{K} (1-p-\delta)^{N-K} }{ (p-\delta)^{K} (1-p+\delta)^{N-K} }.
\end{equation}
Our goal is to ensure that the FP/FN ratios $\alpha_\textrm{FP}, \alpha_\textrm{FN} \leq \alpha$ for a given threshold $\alpha > 0$, which is called the desired significance level.\footnote{We choose the same threshold for $\alpha_\textrm{FP}$ and $\alpha_\textrm{FN}$ for simplicity. The method also applies to the case where two different thresholds for $\alpha_\textrm{FP}$ and $\alpha_\textrm{FN}$ are required (see~\cite{sen2004statistical}).}
By sequential probability ratio tests~\cite{casella2002statistical}, it suffices to keep on drawing samples and stop to make a statistical assertion when either of the conditions on the right-hand-side of the following equation is satisfied:
\begin{equation} \label{eq:sprt_test}
\mathscr{A} \big(K, N) = \begin{cases}
	H_\textrm{null}, &\text{ if } \lambda(K,N) \geq \frac{1 - \alpha}{\alpha}, \\
	H_\textrm{alt}, &\text{ if } \lambda(K,N) \leq \frac{\alpha}{1 - \alpha}.
\end{cases}
\end{equation}
As $N \to \infty$, by the binomial distribution, we have $\lambda(K,N) \to 0$ if $H_\textrm{null}$ holds or $\lambda(K,N) \to \infty$ if $H_\textrm{alt}$ holds, so the above procedure stops with probability $1$. This procedure can be implemented incrementally by Algorithm~\ref{alg:1}.

\begin{algorithm}[!t]

\caption{Statistical model checking of $\mathbb{P}_{\sigma \sim \mathcal{S}} (\sigma \models \varphi) < p$.\label{alg:1}}

\begin{algorithmic}[1]
	\Require Probabilistic model $\mathcal{S}$, desired significance level $\alpha$, and indifference parameter $\delta$.
	
	\State $N \gets 0$, $K \gets 0$, $\lambda \gets 1$.
	
	\While{True}
	
	\State Draw a new sample signal $\sigma$ from $\mathcal{S}$.
	
	\State $K \gets K + \varphi(\sigma)$, $N \gets N + 1$.
	
	\State $\lambda \gets \lambda \frac{ (p+\delta)^{\varphi(\sigma)} (1-p-\delta)^{1-\varphi(\sigma)} }{ (p-\delta)^{\varphi(\sigma)} (1-p+\delta)^{1-\varphi(\sigma)} }$ .
	
	\If {$\lambda \geq \frac{\alpha}{1 - \alpha}$} Return $H_\textrm{null}$
	
	\ElsIf {$\lambda \leq \frac{1 - \alpha}{\alpha}$} Return $H_\textrm{alt}$

	\Else \ Continue

	\EndIf 

	\EndWhile
	
\end{algorithmic}
\end{algorithm}

\begin{remark} \label{rem:2}
By Assumption~\ref{as:indifference}, we do not distinguish between checking $p_\varphi > p$ or checking $p_\varphi \geq p$ in~\eqref{eq:problem 1}. In addition, by the semantics of STL in Section~\ref{sec:prelim}, checking $p_\varphi < p$ or $p_\varphi \leq p$ is equivalent to checking $p_{\neg \varphi} \geq 1 - p$ or $p_{\neg \varphi} > 1 - p$. Thus, the method for checking $p_\varphi > p$ applies to the other three cases.
\end{remark}

==> privacy.tex <==
\section{Differential Privacy in Statistical Model Checking} \label{sec:differential privacy}


Statistical model checking of the probabilistic model $\mathcal{S}$ of an ensemble of cyber-physical systems, e.g., autonomous cars, service robots, and wearable devices, requires analyzing their signals and raises privacy concerns for consumer-level applications. 
It has been shown that even when data is protected using traditional methods such as encryption and occlusion before being processed by an algorithm, an intruder may still be able to infer them by observing the algorithm's output on differing but highly similar data \cite{narayanan2008robust, mandl2021hipaa}. In this section, we recall the widely used notion of differential privacy and demonstrate that it falls short from being applicable for the data sampled by statistical model checking algorithms with their sequential decision-making behavior.


\subsection{Standard differential privacy for sequential algorithms} 
\label{sub:differential privacy}

We denote the statistical model checking Algorithm~\ref{alg:1} by $\mathscr{A}$. The algorithm $\mathscr{A}$ is sequential: it samples signals $\sigma_1, \sigma_2, \ldots$ from the probabilistic model $\mathcal{S}$ until its termination condition is satisfied. Namely, it stops after a sampled data-dependent number of iterations $\tau_\mathscr{A} \in \nat$ and results in an output $o_\mathscr{A} $. With a slight abuse of notation, for an input sequence of sampled signals $\sigma_{1:\infty} = (\sigma_1, \sigma_2, \ldots)$, we write the termination step and output as functions of $\sigma_{1:\infty}$ by $\tau_\mathscr{A}  (\sigma_{1:\infty})$ and $o_\mathscr{A}  (\sigma_{1:\infty})$, respectively. 


Differential privacy aims to prevent malicious inference on $\sigma_{1:\infty}$. Roughly, Algorithm $\mathscr{A}$ is differentially private if an attacker cannot infer the value of $\sigma_i$ even if they can observe $(\tau_\mathscr{A} (\sigma_{1:\infty}), o_\mathscr{A}  (\sigma_{1:\infty}))$ and the values of the rest of the entries $\sigma_{-i}$ of $\sigma_{1:\infty}$, for any sequence $\sigma_{1:\infty}$ and entry $\sigma_i$ in $\sigma_{1:\infty}$.~\cite{dwork2008differential}. Clearly, for a deterministic Algorithm $\mathscr{A}$, the value of $\sigma_i$ can be inferred when the inverse of $\tau_\mathscr{A} (\cdot)$ and $o_\mathscr{A} (\cdot)$ is unique after knowing the value of $\sigma_{-i}$. 


A common approach to achieve differential privacy is to randomize Algorithm $\mathscr{A}$, such that even for the same input sequence $\sigma_{1:\infty}$, the algorithm is randomly executed in slightly different ways and yields different observations. For a randomized algorithm $\mathscr{B}$ of $\mathscr{A}$, although the randomization prevents the intruder to take the inverse of $\tau_{\mathscr{B}} (\cdot)$ and $o_{\mathscr{B}} (\cdot)$, the intruder can still infer the value of $\sigma_i$ by observing the difference in $\tau_{\mathscr{B}}  (\sigma_{1:\infty})$ and $o_{\mathscr{B}}  (\sigma_{1:\infty})$ when the value of $\sigma_{-i}$ is fixed and only the value of $\sigma_i$ changes. To measure the distance between two sequences, we recall the definition of Hamming distance. 


\begin{definition}
The Hamming distance between two input sequences $\sigma_{1:\infty}$ and $\sigma_{1:\infty}'$ is
$D_H (\sigma_{1:\infty},  \sigma_{1:\infty}') = n$ if and only if they are different in only $n \in \mathbb{N}$ entries. Namely, there exists indexes $1 \leq i_1 < \ldots < i_n \in \mathbb{N}$ such that
\begin{equation*}
\begin{cases}
\sigma_j \neq \sigma_j', & \text{ if } j \in \{i_1, \ldots, i_n\} \\
\sigma_j = \sigma_j', & \text{ otherwise.} 
\end{cases}
\end{equation*}
We call two input sequences $\sigma_{1:\infty}$ and $\sigma_{1:\infty}'$ adjacent if $D_H (\sigma_{1:\infty}, \sigma_{1:\infty}') = 1$.
\end{definition}


Differential privacy requires a bound on the worst case change in the probabilities of the random observations for two adjacent input sequences. If the change in distribution is smaller, then it is harder for the intruder to infer the change in the input. We apply the standard notion of differential privacy in \cite{dwork2008differential} to Algorithm~\ref{alg:1} of Section~\ref{sec:prelim} in the following definition.


\begin{definition} \label{def:differential privacy}
A randomized sequential algorithm $\mathscr{B}$ is $\varepsilon$-differentially private, if it holds that
\begin{align} 
&\mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}), o_{\mathscr{B}} (\sigma_{1:\infty}) \big) \in \mathcal{O} \Big) \notag
\\ &\leq e^{\varepsilon} \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}'), o_\mathscr{A} (\sigma_{1:\infty}') \big) \in \mathcal{O} \Big) \label{eq:standard differential privacy}
\end{align}
for any two adjacent input sequences $\sigma_{1:\infty}$ and $\sigma_{1:\infty}'$ and any $\mathcal{O} \subseteq \mathbb{N} \times \{H_\textrm{null}, H_\textrm{alt}\}$. 
\end{definition}

The notation $\mathbb{P}_{\mathscr{B}}$ indicates that the probability is taken from the randomized algorithm $\mathscr{B}$. Similar to the standard definition of differential privacy, Definition~\ref{def:differential privacy} has the following statistical properties. First, if Algorithm $\mathscr{B}$ is differentially private, we can prove the more general statement: for any two non-adjacent input sequences $\sigma_{1:\infty}$ and $\sigma_{1:\infty}'$,
\begin{align}
& \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}), o_{\mathscr{B}} (\sigma_{1:\infty}) \big) \in \mathcal{O} \Big) \leq \notag 
\\ & \quad e^{\varepsilon D_H (\sigma_{1:\infty}, \sigma_{1:\infty}')} \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}'), o_{\mathscr{B}} (\sigma_{1:\infty}') \big) \in \mathcal{O} \Big). \label{eq:prop 0}
\end{align}
In addition, differential privacy bounds the difference in probabilities via their probability ratios, which are commonly used statistics for probabilistic inference. This bound implies that any two input sequences give exactly the same set of observations with non-zero probabilities. Formally, the condition~\eqref{eq:prop 0} implies a necessary condition for differential privacy: 
\begin{align} 
&\mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}), o_{\mathscr{B}} (\sigma_{1:\infty}) \big) \in \mathcal{O} \Big) \neq 0 \notag
\\ & \Longleftrightarrow \mathbb{P}_{\mathscr{B}} \Big( \big( \tau_{\mathscr{B}} (\sigma_{1:\infty}'), o_{\mathscr{B}} (\sigma_{1:\infty}') \big) \in \mathcal{O} \Big) \neq 0. \label{eq:prop 1}
\end{align}
Since most statistical inference methods depend on probability ratios, the condition~\eqref{eq:prop 0} of differential privacy implies that statistical inference for the data is not easy (e.g., lower bounds on the variance of unbiased estimators~\cite{wang2017differentiala}).


By Definition~\ref{def:differential privacy}, the sequential statistical model checking Algorithm~\ref{alg:1} is not differentially private, since for any fixed input sequence $\sigma_{1:\infty}$, its termination time and output $\big( \tau_\mathscr{A} (\sigma_{1:\infty}), o_\mathscr{A} (\sigma_{1:\infty}) \big)$ are deterministic. That does not satisfy the necessary condition of differential privacy~\eqref{eq:prop 1}. 


\subsection{Challenges in achieving standard differential privacy by exponential mechanism} 
\label{sub:Laplace}

The standard approach to make deterministic algorithms differentially private is to randomize their outputs by the exponential algorithm~\cite{mcsherry2007mechanism}. However, we show below that the exponential algorithm cannot achieve the differential privacy from Definition~\ref{def:differential privacy} for the statistical model checking method shown in Algorithm~\ref{alg:1}.

For simplicity, consider only the observation of the termination time $\tau_\mathscr{A} (\sigma_{1:\infty})$. We can define the sensitivity of termination time to changes in any single entry by 
\begin{equation}
\delta_{\tau_\mathscr{A}} := \max_{D_H (\sigma_{1:\infty}, \sigma_{1:\infty}') = 1} \big| \tau_\mathscr{A} (\sigma_{1:\infty}) - \tau_\mathscr{A} (\sigma_{1:\infty}') \big|,
\end{equation}
i.e., the maximal difference in termination time for any two adjacent input sequences of sample signals $\sigma_{1:\infty}$ and $\sigma_{1:\infty}'$. 


If the sensitivity $\delta_{\tau_\mathscr{A}}$ is finite, then the following exponential algorithm achieves differential privacy. The exponential mechanism states that  randomizing algorithm $\mathscr{A}$ to $\mathscr{B}$ such that the probability of terminating at step $k$ is 
\begin{equation} \label{eq:exponential mechanism}
\mathbb{P}_{\mathscr{B}} (\tau_{\mathscr{B}} = k) = \frac{e^{- \varepsilon |\tau_\mathscr{A} - k| / \delta_{\tau_\mathscr{A}}}}{\sum_{h \in \mathcal{H}} e^{- \varepsilon |\tau_\mathscr{A} - h| / \delta_{\tau_\mathscr{A}}}},
\end{equation}
where $\mathcal{H} \subseteq \nat$ is the set of possible values of $\mathscr{A}$, and $\mathbb{P}_{\mathscr{B}}$ means that the randomness should come from the algorithm $\mathscr{B}$ itself. The exponential mechanism~\eqref{eq:exponential mechanism} is $2 \varepsilon$-differentially private~\cite{mcsherry2007mechanism}, since for any two adjacent $\sigma_{1:\infty}$ and $\sigma_{1:\infty}'$, it holds by the definition of sensitivity that for any $k \in \nat$,
\begin{equation} \label{eq:1}
\frac{e^{- \varepsilon  |\tau_\mathscr{A} (\sigma_{1:\infty}) - k| / \delta_{\tau_\mathscr{A}}}}{e^{- \varepsilon  |\tau_\mathscr{A} (\sigma_{1:\infty}') - k| / \delta_{\tau_\mathscr{A}}}} \leq e^{\varepsilon |\tau_\mathscr{A} (\sigma_{1:\infty}) - \tau_\mathscr{A} (\sigma_{1:\infty}')| / \delta_{\tau_\mathscr{A}}} \leq e^{\varepsilon},
\end{equation}
where the first inequality holds by applying the triangle inequality. Since~\eqref{eq:1} holds for any $k$, we have
\begin{equation} \label{eq:2}
\frac{\sum_{h \in \mathcal{H}} e^{- \varepsilon  |\tau_\mathscr{A} (\sigma_{1:\infty}) - h| / \delta_{\tau_\mathscr{A}}}}{\sum_{h \in \mathcal{H}} e^{- \varepsilon  |\tau_\mathscr{A} (\sigma_{1:\infty}') - h| / \delta_{\tau_\mathscr{A}}}} \leq e^\varepsilon.
\end{equation}
Thus, the probability ratio satisfies
\begin{equation} \label{eq:3}
\frac{\mathbb{P}_{\mathscr{B}} \big( \tau_{\mathscr{B}}(\sigma_{1:\infty}) = k \big)}{\mathbb{P}_{\mathscr{B}} \big( \tau_{\mathscr{B}}(\sigma_{1:\infty}') = k \big)} \leq e^{2 \varepsilon}.
\end{equation}


The above technique depends critically on the boundedness of the sensitivity $\delta_{\tau_\mathscr{A}}$, which is generally true for non-sequential algorithms~\cite{mcsherry2007mechanism}. However, this condition is violated for Algorithm~\ref{alg:1}, as shown in Example~\ref{ex:counter}.

\begin{example} \label{ex:counter}
Consider two adjacent input sequences of sample signals with
$$\varphi\big(\sigma_{1:\infty}\big) = (\overbrace{1, \ldots, 1}^{K_1}, \boxed{1},0,1,0, \ldots)$$
and
$$\varphi\big(\sigma_{1:\infty}'\big) = (\overbrace{1, \ldots, 1}^{K_1},\boxed{0},0,1,0, \ldots)$$
in Algorithm~\ref{alg:1}, where $K_1$ satisfies
\begin{equation} \label{eq:K_1}
\frac{ (p+\delta)^{K_1 + 1} }{ (p-\delta)^{K_1 + 1} } \geq \frac{1 - \alpha}{\alpha}, \qquad \frac{ (p+\delta)^{K_1} }{ (p-\delta)^{K_1} } < \frac{1 - \alpha}{\alpha}.
\end{equation}
Recall from equation~\eqref{eq:varphi} that $\varphi(\sigma_i) = 1$ if $\sigma_i \models \varphi$ and $\varphi(\sigma_i) = 0$ if $\sigma_i \not\models \varphi$. By the definition of $\lambda$ in equation~\eqref{eq:probability_ratio}, Algorithm~\ref{alg:1} stops at $\tau_\mathscr{A} (\sigma) = K_1 + 1$ for the input sequence of sample signals $\sigma_{1:\infty}$, and it stops at $\tau_\mathscr{A} (\sigma') = \infty$ for the other input sequence of sample signals $\sigma'_{1:\infty}$. This shows that the sensitivity $\delta_{\tau_\mathscr{A}} = \infty$ and the exponential mechanism cannot achieve $\varepsilon$-differential privacy for any finite $\varepsilon$. Finally, we note that the case of $\tau_\mathscr{A} (\sigma') = \infty$ happens with probability $0$, thus it does not violate the fact that the algorithm $\mathscr{A}$ stops almost surely with probability $1$.
\end{example}
